Graph-Based Operator Learning from Limited Data on Irregular Domains

Operator learning seeks to approximate mappings from input functions to output solutions, particularly in the context of partial differential equations (PDEs). While recent advances such as DeepONet and Fourier Neural Operator (FNO) have demonstrated strong performance, they often rely on regular grid discretizations, limiting their applicability to complex or irregular domains. In this work, we propose a Graph-based Operator Learning with Attention (GOLA) framework that addresses this limitation by constructing graphs from irregularly sampled spatial points and leveraging attention-enhanced Graph Neural Netwoks (GNNs) to model spatial dependencies with global information. To improve the expressive capacity, we introduce a Fourier-based encoder that projects input functions into a frequency space using learnable complex coefficients, allowing for flexible embeddings even with sparse or nonuniform samples. We evaluated our approach across a range of 2D PDEs, including Darcy Flow, Advection, Eikonal, and Nonlinear Diffusion, under varying sampling densities. Our method consistently outperforms baselines, particularly in data-scarce regimes, demonstrating strong generalization and efficiency on irregular domains.

==> abstract.tex <==
\begin{abstract}
Operator learning seeks to approximate mappings from input functions to output solutions, particularly in the context of partial differential equations (PDEs). While recent advances such as DeepONet and Fourier Neural Operator (FNO) have demonstrated strong performance, they often rely on regular grid discretizations, limiting their applicability to complex or irregular domains. In this work, we propose a \textbf{G}raph-based \textbf{O}perator \textbf{L}earning with \textbf{A}ttention (GOLA) framework that addresses this limitation by constructing graphs from irregularly sampled spatial points and leveraging attention-enhanced Graph Neural Netwoks (GNNs) to model spatial dependencies with global information. To improve the expressive capacity, we introduce a Fourier-based encoder that projects input functions into a frequency space using learnable complex coefficients, allowing for flexible embeddings even with sparse or nonuniform samples. We evaluated our approach across a range of 2D PDEs, including Darcy Flow, Advection, Eikonal, and Nonlinear Diffusion, under varying sampling densities. Our method consistently outperforms baselines, particularly in data-scarce regimes, demonstrating strong generalization and efficiency on irregular domains.

\end{abstract}

==> analysis.tex <==
\section{Theoretical Analysis}
\label{theory}
Following the universal approximation theorem for operators \citep{lu2019deeponet}, neural operator architectures can approximate any continuous operator $\mathcal{G}$ between Banach spaces when provided with sufficient capacity. 

\paragraph{Proposition.} Let $\mathcal{G}: \mathcal{F} \rightarrow \mathcal{U}$ be a continuous nonlinear operator between separable Banach spaces. Then, under sufficient model capacity, the GOLA architecture $\mathcal{G}_\theta$ can approximate $\mathcal{G}$ arbitrarily well in the $L^2(\Omega)$ norm over a compact domain $\Omega$, i.e.,
$\sup_{f \in \mathcal{F}_\delta} \| \mathcal{G}(f) - \mathcal{G}_\theta(f) \|_{L^2(\Omega)} < \epsilon$,
for any $\epsilon > 0$ and compact subset $\mathcal{F}_\delta \subset \mathcal{F}$.



\textit{Proof}. Given a function $f \in \mathcal{F} \subset L^2(\Omega)$, we sample it at $N$ spatial locations $\{x_i\}_{i=1}^N \subset \Omega$ to obtain a discrete representation $f_N = (f(x_1), \ldots, f(x_N)) \in \mathbb{R}^N.$
Since $\Omega$ is compact, by increasing $N$ the point cloud $\{x_i\}$ becomes dense in $\Omega$. Thus, $f_N$ can approximate $f$ arbitrarily well in $L^2(\Omega)$ norm via interpolation over the sampling set.

Define a set of complex Fourier basis functions $\{\phi_m(x) = e^{2\pi i \langle \omega_m, x \rangle}\}_{m=1}^M$. The Fourier basis is complete in $L^2(\Omega)$, so for any $f \in \mathcal{F}$ and $\delta > 0$, there exists $M$ such that
\begin{align*}
    \left\| f(x) - \sum_{m=1}^M \hat{f}_m \phi_m(x) \right\|_{L^2(\Omega)} < \delta.
\end{align*}

This guarantees that the learnable Fourier encoder in GOLA can approximate the functional input $f$ to arbitrary precision.

Construct a graph $G=(V, E)$ with node set $V=\{x_i\}_{i=1}^N$, where edges encode local spatial relationships. 
According to universal approximation results for GNNs \citep{xu2019powerful}, \citep{morris2019weisfeiler}, for any continuous function defined on graphs, a GNN with sufficient depth and width can approximate it arbitrarily well. Thus, the GNN decoder can approximate the mapping from input features to solution values
\begin{align*}
    (f(x_1), \dots, f(x_N)) \mapsto (\mathcal{G}(f)(x_1), \dots, \mathcal{G}(f)(x_N))
\end{align*}

Let $\mathcal{T}_N$ denote the sampling operator, $\mathcal{F}_\theta$ the Fourier encoder, and $\mathcal{D}_\theta$ the GNN decoder. Then the GOLA operator can be written as
\begin{align*}
    \mathcal{G}_\theta = \mathcal{D}_\theta \circ \mathcal{F}_\theta \circ \mathcal{T}_N
\end{align*}
Each component is continuous and approximates its target arbitrarily well. Since composition of continuous approximations preserves continuity, and $\mathcal{F}_\delta$ is compact, the total approximation error can be made less than any $\varepsilon > 0$ by choosing $N$, $M$, and model capacity large enough such that
\begin{align*}
    \sup_{f \in \mathcal{F}_\delta} \| \mathcal{G}(f) - \mathcal{G}_\theta(f) \|_{L^2(\Omega)} < \varepsilon
\end{align*}




==> checklist.tex <==

\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See abstract and introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Limitation in Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Theoretical Analysis.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: \justificationTODO{}
    \item[] Guidelines: We don't open it now.
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use different seed to test.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Societal Impact in Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper doesn't have such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have cited the original paper about the models that we use.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not include any experiments and research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The core method development in this research does not involve LLMs as any important, original, or non-standard components.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> conclusion.tex <==
\section{Conclusion}

We introduce a \textbf{G}raph-based \textbf{O}perator \textbf{L}earning with \textbf{A}ttention (GOLA) framework, that effectively models PDE solution operators on irregular domains using attention-enhanced graph neural networks and a Fourier-based encoder. Through comprehensive experiments across diverse PDE benchmarks including Darcy Flow, Advection, Eikonal, and Nonlinear Diffusion, GOLA consistently outperforms baselines particularly in data-scarce regimes and under severe resolution shifts. 
We demonstrate GOLA’s superior generalization, resolution scalability, and robustness to sparse sampling.
These results highlight the potential of combining spectral encoding and localized message passing with attention to build continuous, data-efficient operator approximators that adapt naturally to non-Euclidean geometries. This study demonstrates that graph-based representations provide a powerful and flexible foundation for advancing operator learning in real-world physical systems with irregular data.



==> exp.tex <==
\section{Experiments}
We evaluate the proposed model GOLA on four 2D PDE benchmarks including Darcy Flow, Nonlinear Diffusion, Eikonal, and Advection.
For each dataset, we simulate training data with 5, 10, 20, 30, 40, 50, 80, 100 samples and use 100 examples for testing.
To construct graphs, we randomly sample 20, 30, 40, 50, 60, 70, 80, 90, 100, 200, 300, 400, 500, 600, 700, 800, 900, 1000 points from a uniform \( 128 \times 128 \) grid over the domain \([0, 1] \times [0, 1]\). The sampled points define the nodes of the graph.
Our model learns to approximate the solution operator from these irregularly sampled inputs. We aim to test generalization under both limited data and resolution changes.
We compare against the following baselines including DeepONet, FNO, Graph Convolutional Network (GCN), and Graph Kernel Network (GKN).
We test DeepONet, FNO, GCN on standard grid data, and test GKN and our model GOLA on 1000 sample data randomly selected from grid data. 

% \textbf{Performance Across PDEs.} GOLA consistently achieves lower test errors across all PDEs and training regimes. For example, with 100 training samples and a test density of 1000, GOLA achieves a test error of 0.0741 for Darcy flow and 0.0302 for Nonlinear Diffusion—surpassing GKN by margins of $57.6\%$ and $28.9\%$, respectively. The improvements are particularly significant in Eikonal and Diffusion problems, which benefit from GOLA’s ability to model both local and global dependencies.



% \textbf{Data Efficiency.} In low-data regimes $N_{tr} \leq 20$, GOLA shows strong generalization. With only 10 training examples, it reduces Eikonal error from 0.1956 (GKN) to 0.1286, and Diffusion error from 0.2346 to 0.1204. Compared to GCN and DeepONet, our model provides over $50\%$ error reduction on several benchmarks even with minimal supervision, confirming its effectiveness as a data-efficient operator learner.


%  \textbf{Resolution Generalization.} A defining feature of operator learning is the ability to generalize to unseen spatial resolutions. We test GOLA’s predictions on finer test sets while training on coarse data. As shown in Table 3 and Figure 5, the test error on Nonlinear Diffusion drops from 0.0945 (density 100) to 0.0415 (density 4000), even without retraining. This supports the model’s ability to learn a resolution-invariant solution operator, critical for physical systems with varying mesh fidelity.



%  \textbf{Error Reduction Compared to GKN.} Tables 17–27 report detailed comparisons between GOLA and GKN across multiple training sizes and densities. GOLA outperforms GKN in all scenarios:
% \begin{itemize}
% \item \textbf{Eikonal and Diffusion}: Largest gains, with up to $58\%$ test error reduction, even at moderate densities (e.g., density = 600, $N_{tr}=40$).
% \item \textbf{Darcy Flow}: Error reduced from 0.1748 (GKN) to 0.0741, a $57.6\%$ improvement at full training size.
% \item \textbf{Advection}: Gains range from $10-46\%$, with stronger improvements at low sample density.
% \end{itemize}

% \textbf{Sparse Sampling Robustness.} Even under extremely sparse test-time sampling (e.g., 20 points out of $128 \times 128$), GOLA performs reliably. At sampling density 20, training size 100, compared to GKN, GOLA achieves:
% \begin{itemize}
% \item $15.1\%$ lower error on Darcy flow,
% \item $55.9\%$ on Advection,
% \item $31.6\%$ on Eikonal, and
% \item $15.7\%$ on Diffusion,
% \end{itemize}
% This indicates strong inductive bias and robustness to partial observations, crucial for real-world applications like sensor networks or adaptive simulations.

% \textbf{Summary.} GOLA exhibits superior performance in all key operator learning criteria: generalization from limited data, handling of irregular sampling, resolution scalability, and robustness to sparse observations. Its attention-enhanced graph architecture, coupled with Fourier-based encoding, offers a principled way to learn continuous solution operators across diverse geometries and regimes.


\textbf{Comparison with baselines.} From Table \ref{fig:comparison_baseline}, we test on 30 training data, our model consistently achieves the lowest test error across all four benchmarks. For example, in Darcy Flow, GCN whose relative $L_2$ error is 1.3902 performs the worst, suggesting graph-only models may lack the expressiveness needed here. FNO and GKN improve significantly whose relative $L_2$ error are 0.1678 and 0.2375 respectively, showing the benefit of spectral and kernel-based methods. GOLA further improves performance with a relative $L_2$ error 0.1554. From Table \ref{tab:error_reduction}, we use 100 training data, and 1000 sample points. It shows that our method GOLA outperforms GKN across all four datasets Darcy Flow, Advection, Eikonal, Nonlinear Diffusion with error reduction $34.38\%, 20.65\%, 47.69\%, 57.95\%$ respectively.
In Figure \ref{fig:test-errors-train-all}, we display test error comparisons across four PDE benchmarks for five different models. GCN struggles across all PDEs, especially as data decreases. DeepONet and FNO show stronger performance, particularly with more data. GKN and GOLA are more data-efficient. And GOLA generalizes best under limited training samples, across all four PDE types.
In Figure \ref{fig:heatmaps_train_sizes}, we present heatmaps of error reduction across different PDE benchmarks under varying training data sizes and sample densities. Nonlinear Diffusion consistently shows the highest error reduction across all training sizes and densities. And it becomes more prominent at high sample densities even under very small training sizes such as 10.



\begin{table}[H]
\centering
\caption{\small \textit{Test errors for different models trained on 30 training data samples across various PDE benchmarks}}
\label{fig:comparison_baseline}
\small
\begin{tabular}{lccccc}
\toprule
\textit{Dataset} & GCN & DeepONet & FNO & GKN & Ours \\
\midrule
Darcy Flow & 1.3902 & 0.4163 & 0.1678 & 0.2375 & 0.1554 \\
Advection & 0.9620 & 0.3925 & 0.3873 & 0.5353 & 0.3707 \\
Eikonal & 0.2120 & 0.1442 & 0.0874 & 0.1530 & 0.0803 \\
Nonlinear Diffusion & 0.2703 & 0.2468 & 0.0793 & 0.1520 & 0.0747 \\
\bottomrule
\end{tabular}
\end{table}


\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/baselines_with_train_100.jpg}
        % \caption{Train Size = 100}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/baselines_with_train_50.jpg}
        % \caption{Train Size = 50}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/baselines_with_train_40.jpg}
        % \caption{Train Size = 40}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/baselines_with_train_30.jpg}
        % \caption{Train Size = 30}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/baselines_with_train_20.jpg}
        % \caption{Train Size = 20}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/baselines_with_train_10.jpg}
        % \caption{Train Size = 10}
    \end{subfigure}
    
    \caption{\small \textit{Test errors across PDE benchmarks with varying training data sizes}}
    \label{fig:test-errors-train-all}
\end{figure}


\begin{table}[H]
\centering
\caption{\small \textit{Comparison of GKN and GOLA with sample density=1000, train data size=100}}
\label{tab:error_reduction}
\small
\begin{tabular}{lccc}
\toprule
\textit{Dataset} & GKN & Ours & Error Reduction \\
\midrule
Darcy Flow & 0.1748 & 0.1147 & 34.38\% \\
Advection & 0.2886 & 0.2290 & 20.65\% \\
Eikonal & 0.1168 & 0.0611 & 47.69\% \\
Nonlinear Diffusion & 0.1044 & 0.0439 & 57.95\% \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure}[htbp]
    \centering

    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/error_heatmap_with_train_100.jpg}
        % \caption{Train Size = 100}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/error_heatmap_with_train_50.jpg}
        % \caption{Train Size = 50}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/error_heatmap_with_train_40.jpg}
        % \caption{Train Size = 40}
    \end{subfigure}

    \vskip\baselineskip

    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/error_heatmap_with_train_30.jpg}
        % \caption{Train Size = 30}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/error_heatmap_with_train_20.jpg}
        % \caption{Train Size = 20}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/error_heatmap_with_train_10.jpg}
        % \caption{Train Size = 10}
    \end{subfigure}
    \caption{\small \textit{Error reduction heatmaps across training data sizes and sample densities for PDE Benchmarks}}
    \label{fig:heatmaps_train_sizes}
\end{figure}







\textbf{Generalization across sample densities.}
From Table \ref{tab:Test_errors_test_sampling_densities}, we use 100 training data, and choose three types of sampling densities 20, 500, 1000 which represent small, medium and high sample densities. We can conclude that increasing sample density leads to smaller test error.
\begin{table}[H]
        \centering
    \caption{ \small \textit{Test errors for small, medium, and high sampling densities with training data size=100}}
    \small
    \label{tab:Test_errors_test_sampling_densities}
    \begin{tabular}{lccc}
        \toprule
        \text{\textit{Sample Density}} & \text{20} & \text{500} & \text{1000} \\
        \midrule
        Darcy Flow       & 0.4269 & 0.1433 & 0.1147 \\
        Advection  & 0.3980 & 0.2462 & 0.2290 \\
        Eikonal         & 0.1236 & 0.0671 & 0.0611 \\
        Nonlinear Diffusion  & 0.2030 & 0.0637 & 0.0439 \\
        \bottomrule
    \end{tabular}
\end{table}


\textbf{Resolution generalization.} From Table \ref{tab:vary_test_pts} and Figure \ref{fig:test-error-test}, we use 100 training data and sample 1000 training sample points, then we test the relative $L_2$ error in different test sample densities 100, 500, 1000, 2000, 4000. It shows that the test error decreases as test sample density increases, suggesting that the model generalizes better when evaluated on finer-resolution grids even though it is trained on a coarser sampling.

\begin{table}[H]
    \centering
    \caption{ \small\textit{Test errors for different test sampling densities with training sample density=1000}}
    \label{tab:vary_test_pts}
    \small
    \begin{tabular}{lccccc}
        \toprule
        % \textit{Dataset}      & \multicolumn{4}{c}{Test Sample Points} \\
        % \cmidrule(lr){2-5}
        \text{\textit{Test Sample Density}}                      & 100     & 500     & 1000    & 2000 & 4000    \\
        \midrule
        Darcy Flow            & 0.2419  & 0.1304  & 0.1147  & 0.0990  & 0.0913  \\
        Advection             & 0.3757  & 0.2535  & 0.2290  & 0.2239  & 0.2181  \\
        Eikonal               & 0.0819  & 0.0687  & 0.0611  & 0.0610  & 0.0604  \\
        Nonlinear Diffusion   & 0.0945  & 0.0501  & 0.0439  & 0.0417  & 0.0415  \\
        \bottomrule
    \end{tabular}
\end{table}


\begin{figure}[H]
    \centering
    \begin{minipage}[b]{0.48\linewidth}
        \centering
    \includegraphics[width=\linewidth]{figures/train_points1000_with_test.jpg}
    \caption{\small \textit{Test error trend with test sample density}}
    \label{fig:test-error-test}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.48\linewidth}
        \centering
    \includegraphics[width=\linewidth]{figures/test_points4000_with_training_size.jpg}
    \caption{\small \textit{Test error trend with train data size}}
    \label{fig:test-error-train}
    \end{minipage}
\end{figure}




\textbf{Data Efficiency.} From Table \ref{tab:test-trend-train} and Figure \ref{fig:test-error-train}, we use 4000 sample points and change different training data size to test the performance.
The error for Darcy Flow drops from 0.2005 to 0.0724, and the rapid improvement from 20 to 40 samples, then smaller incremental gains suggests the model captures the key inductive bias early.
The error for Eikonal decreases from 0.1112 to 0.0667, which is a moderate and smooth decline, indicating stable generalization.
In Figure \ref{fig:Test-error-sample}, it shows the test error for four PDE benchmarks as a function of training data size, under different test point resolutions.All PDEs generally show decreasing test error as the training data size increases, confirming that more training data improves generalization. Eikonal and Nonlinear Diffusion achieve good accuracy with very small training sets, suggesting these tasks require fewer data to generalize well. For Darcy Flow and Advection, the errors decrease more sharply with smaller training data sizes compared to larger ones which indicates that our model is more data-efficient in the data-scarce regime.


\begin{table}[H]
        \centering
    \caption{ \small \textit{Test errors under varying numbers of training data size with sample density=4000} }
    \small
    \label{tab:test-trend-train}
    \begin{tabular}{lccccc}
        \toprule
        % \multicolumn{6}{c}{\textit{sample density} = 4000} \\
        % \midrule
        \textit{Training data size} & 20     & 40     & 60     & 80     & 100    \\
        \midrule
        Darcy Flow        & 0.2005 & 0.1112 & 0.0905 & 0.0863 & 0.0724 \\
        Advection    & 0.4790 & 0.3381 & 0.3184 & 0.2380 & 0.1952 \\
        Eikonal          & 0.1112 & 0.0934 & 0.0762 & 0.0673 & 0.0667 \\
        Nonlinear Diffusion    & 0.0599 & 0.0400 & 0.0342 & 0.0312 & 0.0302 \\
        \bottomrule
    \end{tabular}
\end{table}







% \begin{figure}[htbp]
%     \centering

%     \begin{subfigure}[b]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/baselines_with_train_100.jpg}
%         % \caption{Train Size = 100}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/baselines_with_train_50.jpg}
%         % \caption{Train Size = 50}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/baselines_with_train_40.jpg}
%         % \caption{Train Size = 40}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/baselines_with_train_30.jpg}
%         % \caption{Train Size = 30}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/baselines_with_train_20.jpg}
%         % \caption{Train Size = 20}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/baselines_with_train_10.jpg}
%         % \caption{Train Size = 10}
%     \end{subfigure}

    
%     \caption{Test errors for different model}
%     \label{fig:Test-errors-for-different-model-subfigures}
% \end{figure}





% \begin{table*}
%         \centering
%     \caption{\small \textit{Test errors with low, medium, and high test sampling densities with training data size=100}}
%     \small
%     \begin{tabular}{lccc}
%         \toprule
%         \text{\textit{Sample Density}} & \text{20} & \text{500} & \text{1000} \\
%         \midrule
%         Darcy Flow       & 0.4269 & 0.1433 & 0.1147 \\
%         Advection  & 0.3980 & 0.2462 & 0.2290 \\
%         Eikonal         & 0.1236 & 0.0671 & 0.0611 \\
%         Nonlinear Diffusion  & 0.2030 & 0.0637 & 0.0439 \\
%         \bottomrule
%     \end{tabular}
% \end{table*}






% \begin{figure}[htbp]
%   \centering
%   \begin{subfigure}[b]{0.45\textwidth}
%     \includegraphics[width=\linewidth]{figures/Test_errors_sampling_densities.jpg}
%     \caption{\small \textit{Test errors with low, medium, and high sampling densities with training data size=100}}
%     \label{fig:sub1}
%   \end{subfigure}
%   \hspace{0.05\textwidth} % horizontal space between the two figures
%   \begin{subfigure}[b]{0.45\textwidth}
%     \includegraphics[width=\linewidth]{figures/Test_errors_test_sampling_densities.jpg}
%     \caption{\small \textit{Test errors with low, medium, and high test sampling densities with training data size=100, train sampling density=1000}}
%     \label{fig:sub2}
%   \end{subfigure}
%   % \caption{Main caption for both figures}
%   \label{fig:main}
% \end{figure}























% \begin{figure}[htbp]
%     \centering

%     \begin{subfigure}[b]{0.32\textwidth}
%         \includegraphics[width=\textwidth]{fig_train100.png}
%         \caption{Train Size = 100}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \includegraphics[width=\textwidth]{fig_train50.png}
%         \caption{Train Size = 50}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \includegraphics[width=\textwidth]{fig_train40.png}
%         \caption{Train Size = 40}
%     \end{subfigure}

%     \caption{Error Reduction Heatmaps (Train Sizes: 100, 50, 40)}
%     \label{fig:heatmaps_row1}
% \end{figure}



\begin{figure}[htbp]
    \centering

    % Top Row
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/test_points900_with_training_size.jpg}
        % \caption{Train Size = 100}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/test_points800_with_training_size.jpg}
        % \caption{Train Size = 50}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/test_points700_with_training_size.jpg}
        % \caption{Train Size = 40}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/test_points600_with_training_size.jpg}
        % \caption{Train Size = 30}
    \end{subfigure}

    \vskip\baselineskip

    % Bottom Row
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/test_points500_with_training_size.jpg}
        % \caption{Train Size = 20}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/test_points400_with_training_size.jpg}
        % \caption{Train Size = 10}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/test_points300_with_training_size.jpg}
        % \caption{Extra 1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/test_points200_with_training_size.jpg}
        % \caption{Extra 2}
    \end{subfigure}
    \caption{\small \textit{Test error trends across varying sample densities for PDE benchmarks}}
    \label{fig:Test-error-sample}
\end{figure}

\textbf{Time Complexity and Memory Cost.} 
We analyze the computational complexity of the GOLA architecture in terms of the number of spatial points $N$, Fourier modes $M$, feature channels $C$, and edges $E \sim \mathcal{O}(Nk) $, where $k$ is the average number of neighbors in the sparse spatial graph.
The time complexity for GOLA is $\mathcal{O}(MNC)+\mathcal{O}(NkC^2)+\mathcal{O}(NkC)$.
The count of parameters for GOLA is 2,900,249.






==> intro.tex <==

\section{Introduction}


Learning mappings between function spaces is a fundamental task in computational physics and scientific machine learning, especially for approximating solution operators of partial differential equations (PDEs). 
 Operator learning offers a paradigm shift by learning the solution operator directly from data, enabling fast, mesh-free predictions across varying input conditions. 
Despite their success, existing operator learning models such as DeepONet \citep{lu2019deeponet} and Fourier Neural Operator (FNO) \citep{li2020fourier} exhibit notable limitations that restrict their applicability in more general settings. A key shortcoming lies in their reliance on regular, uniform grid discretizations. FNO, for instance, requires inputs to be defined on fixed Cartesian grids to leverage fast Fourier transforms efficiently. This assumption limits their flexibility and generalization ability when applied to problems defined on complex geometries, irregular meshes, or unstructured domains, which are common in real-world physical systems. Furthermore, these models often struggle with sparse or non-uniformly sampled data, leading to degraded performance and increased computational cost when adapting to more realistic, heterogeneous scenarios. 

To address these limitations, we propose a \textbf{G}raph-based \textbf{O}perator \textbf{L}earning with \textbf{A}ttention (GOLA) framework that leverages Graph Neural Networks (GNNs) to learn PDE solution operators over irregular spatial domains. By constructing graphs from sampled spatial coordinates and encoding local geometric and functional dependencies through message passing, the model naturally adapts to non-Euclidean geometries.
To enhance global expressivity, we further incorporate attention-based mechanisms that can capture long-range dependencies more effectively and a Fourier-based encoder that projects input functions into a frequency domain using learnable complex-valued bases. 
Our model exhibits superior data efficiency and generalization, achieving smaller prediction errors with fewer training samples and demonstrating robustness under domain shifts.



The main contributions of this work are as follows:
\begin{itemize}
    \item We introduce GOLA, a unified architecture combining spectral encoding and attention-enhanced GNNs for operator learning on irregular domains.
    \item We propose a learnable Fourier encoder that projects input functions into a frequency domain tailored for spatial graphs.
    \item  Through extensive experiments, we demonstrate that GOLA generalizes across PDE types, sample densities, and resolution shifts, achieving state-of-the-art performance in challenging data-scarce regimes.
\end{itemize}













==> method.tex <==

\section{Methodology}

\subsection{Problem Formulation}

% Operator learning aims to approximate a mapping from input parameters and functions to their corresponding output functions. This framework is especially relevant in the context of solving partial differential equations (PDEs), where the goal is to learn the solution operator of a given PDE system.
% Operator learning aims to approximate a mapping from input functions and parameters to their corresponding output functions. This framework is particularly suited for solving partial differential equations (PDEs), where the objective is to learn the solution operator associated with a given PDE system.

Consider the general form of a PDE
\begin{equation}
    \mathcal{N}[u](\mathbf{x}) = f(\mathbf{x}), \quad \mathbf{x} \in \Omega \times [0, \infty)
\end{equation}
where $\mathbf{x}$ denotes a compact representation of the spatial and temporal coordinates, $\Omega$ is the spatial domain, and $[0, \infty)$ is the temporal domain. $\mathcal{N}$ is a differential operator, $u(\mathbf{x})$ is the unknown solution, and $f(\mathbf{x})$ is a given source term.
The objective is to learn the solution operator $\mathcal{G}: \mathcal{F} \to \mathcal{U}$, where $\mathcal{F}$ and $\mathcal{U}$ are Banach spaces.
We assume access to a training dataset $\mathcal{D} = \{ (f_n, u_n) \}_{n=1}^N$, consisting of multiple input-output function pairs, where each $f_n(\cdot)$ and $u_n(\cdot)$ is represented by discrete samples over a finite set of points.

While existing approaches such as DeepONet and FNO have demonstrated strong performance, they typically rely on structured, grid-based discretizations of the domain. This assumption limits their applicability to unstructured meshes, complex geometries, and adaptively sampled domains.
To overcome this limitation, we employ GNNs for operator learning by representing the domain as a graph. This allows for modeling on arbitrary domains and sampling patterns. 
Once trained, the operator learning model can efficiently predict the solution $u$ for a new instance of the input $f$ at random locations.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/model_flow.pdf}  % Adjust path and size
    % \caption{\small \textit{Work Flow}}
    \label{fig:my_pdf}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/model.pdf}  % Adjust path and size
    \caption{\small \textit{GOLA Model}}
\end{figure}



\subsection{Graph Construction}

To represent PDE solutions over irregular domains, we begin by randomly sampling a subset of points $\{x_i\}^N_{i=1}$ from a uniform grid in 2D space. We then construct a graph $G = (V, E)$ with nodes $V=\{x_i\}$ and edges $E$ determined by a radius $r$. Edges are created based on spatial proximity. Two nodes are connected if the Euclidean distance between them is less than a threshold $r$ such that 
  $(i,j) \in E$ if and only if $\| x_i - x_j \|_2 \leq r$.
Each edge $(i, j)$ carries edge attributes $e_{ij}$ that encode both geometric and feature-based information, such as the relative coordinates and function values at nodes $i$ and $j$ such that $e_{ij} = \mathbin\Vert (x_i, x_j, f(x_i), f(x_j))$,
where $\mathbin\Vert$ is the concatenation operation. This graph-based representation allows us to model unstructured spatial domains and enables message passing among nonuniform samples.
% The adjacency matrix $A \in \mathbb{R}^{m \times m}$ is symmetrized and row-normalized as
% \begin{align}
%     \hat{A} = D^{-\frac{1}{2}} (A + I) D^{-\frac{1}{2}}
% \end{align}
% where $D$ is the degree matrix.



\subsection{Fourier Encoder}


We define a set of learnable frequencies
$   \left\{ \omega_m \in \mathbb{R}^2 \,\middle|\, m = 1, \ldots, M \right\}$.


For any coordinate $ x \in \mathbb{R}^2 $, the $m$-th basis function is given by the complex exponential
\begin{align}
    \varphi_m(x) = e^{2\pi i \langle \omega_m, x \rangle}
\end{align}

where $\langle \cdot, \cdot \rangle$ denotes the standard Euclidean inner product, and $i$ is the imaginary unit.


At the discrete level, for a batch of $B$ samples and $N$ points per sample, the basis matrix is defined as
\begin{align}
    \Phi \in \mathbb{C}^{B \times N \times M}, \quad \Phi_{b,i,m} = e^{2\pi i \langle \omega_m, x_i^{(b)} \rangle}
\end{align}
where $x_i^{(b)}$ denotes the $i$-th coordinate point in the $b$-th batch sample.


Given the input $f \in \mathbb{R}^{B \times C_{\text{in}} \times N}$ sampled at points $\{ x_i \}$, we first project onto the Fourier basis.
We compute the Fourier coefficients by
\begin{align}
    \hat{u}_{b,c,m} = \frac{1}{N} \sum_{i=1}^{N} f_{b,c,i} \, \overline{\varphi_m\left(x_i^{(b)}\right)}
\end{align}
where $\overline{(\cdot)}$ denotes complex conjugation.

We introduce a learnable set of complex Fourier coefficients $   W \in \mathbb{C}^{C_{\text{in}} \times C_{\text{out}} \times M}$.
The spectral filtering operation is
\begin{align}
    \hat{v}_{b,o,m} = \sum_{c=1}^{C_{\text{in}}} \hat{u}_{b,c,m} \, W_{c,o,m}
\end{align}


We reconstruct the output in the physical domain by applying the inverse transform
\begin{align}
    v_{b,o,i} = \sum_{m=1}^{M} \hat{v}_{b,o,m} \, \varphi_m\left(x_i^{(b)}\right)
\end{align}


Since $v$ is complex-valued, we only take its real part for the output as $h = \text{Re}(v) \in \mathbb{R}^{B \times C_{\text{out}} \times N}$.
The output $h$ serves as the input node features for the downstream GNN model.



\subsection{Message Passing}

Given a node $i \in V$ and its set of neighbors $\mathcal{N}(i)$, the pre-processed messages $\{ m_{ij} \}_{j \in \mathcal{N}(i)}$ are first computed using a learnable neural network $g_{\Theta}$ as
\begin{align}
  m_{ij} = g_{\Theta}(h_i, h_j, e_{ij})  
\end{align}
where $h_i$ and $h_j$ are node features, and $e_{ij}$ denotes edge attributes.

Then we aggregate message from neighbors such that
\begin{align}
    \hat{m} = \mathbin\Vert (\frac{1}{|\mathcal{N}(i)|} \sum_{j \in \mathcal{N}(i)} m_{ij}, \max_{j \in \mathcal{N}(i)} m_{ij}, \min_{j \in \mathcal{N}(i)} m_{ij},  \sqrt{ \frac{1}{|\mathcal{N}(i)|} \sum_{j \in \mathcal{N}(i)} (m_{ij} - \frac{1}{|\mathcal{N}(i)|} \sum_{j \in \mathcal{N}(i)} m_{ij})^2 })
\end{align}


This concatenated feature vector is processed by a post-aggregation neural network \( \gamma_{\Theta} \) to produce the updated node representation by
\begin{align}
  h_i' = \gamma_{\Theta}\left( h_i, \hat{m} \right)
\end{align}
The updated node representation is passed through additional MLP layers with residual connections to enhance expressiveness.

\subsection{Multi-Head Self-Attention}


We employ $H$ independent attention heads. For each head $h$,
the query, key and value functions are computed as linear projections
\begin{align}
q^{(h)}(x) = W_q h'(x), \quad
k^{(h)}(y) = W_k h'(y), \quad
v^{(h)}(y) = W_v h'(y)
\end{align}
where $W_q, W_k, W_v \in \mathbb{R}^{d_h \times C_{\text{out}}}$, $q^{(h)}(x), k^{(h)}(y), v^{(h)}(y) \in \mathbb{R}^{d_h}$ are learned head-specific features, and $d_h$ is the dimension per attention head.

Before computing attention, the keys and values are normalized
\begin{align}
\tilde{k}^{(h)}(y) = \text{Norm}(k^{(h)}(y)), \quad
\tilde{v}^{(h)}(y) = \text{Norm}(v^{(h)}(y))
\end{align}
where $\text{Norm}(\cdot)$ denotes instance normalization.

We compute
\begin{align}
G_h = \sum_{j=1}^N \tilde{k}^{(h)}(y_j)^\top \tilde{v}^{(h)}(y_j) w(y_j),
\quad
(\mathcal{K}_h h')(x_i) = q^{(h)}(x_i) G_h
\end{align}

% and then
% \begin{align}
% (\mathcal{K}_h h')(x_i) = q^{(h)}(x_i) G_h
% \end{align}


The outputs are concatenated and projected to the output space by
\begin{align}
  (\mathcal{K}h')(x_i) = \mathbin\Vert \left( (\mathcal{K}_1 h')(x_i), \ldots, (\mathcal{K}_H h')(x_i) \right),
\quad
\hat{h}(x_i) = W_{\text{out}} (\mathcal{K}h')(x_i)
\end{align}
where where $G_h \in \mathbb{R}^{d_h \times d_h}$, $w$ is calculated by the number of points, $W_{\text{out}} \in \mathbb{R}^{C_{\text{out}} \times (C_{\text{out}} \cdot H)}$.

The result is then passed through a linear projection layer to update the node features.

\subsection{Message Passing with Attention}
We update node features and add a skip connection by
\begin{align}
  \hat{h}_i' = W_1 \hat{h}_i + \sum_{j \in \mathcal{N}(i)} \alpha_{ij} \left( W_2 \hat{h}_j + W_3 e_{ij} \right),  
  \quad
    \hat{h}_i' = \hat{h}_i' + W_s \hat{h}_i
\end{align}

The attention weights $\alpha_{ij}$ are computed using a scaled dot-product attention mechanism by
\begin{align}
    \alpha_{ij} = \text{softmax}_j \left( \frac{ \left( W_4 \hat{h}_i \right)^\top \left( W_5 \hat{h}_j + W_3 e_{ij} \right) }{ \sqrt{d} } \right)
\end{align}
where $d$ is the dimensionality of the head, and the softmax is applied over the set of neighbors $j \in \mathcal{N}(i)$.
Then we add a linear projection to produce the predicted solution $\hat{u}$.



\subsection{Training}

The model is trained to minimize the relative $L_2$ error between predicted and true solutions by
\begin{align}
    \mathcal{L}_2(\theta) = \frac{ \| u - \mathcal{G}_\theta(f) \|_{L^2(\Omega)} }{ \| u \|_{L^2(\Omega)} }
\end{align}



==> neurips_2025.tex <==
% \documentclass{article}


% % if you need to pass options to natbib, use, e.g.:
% %     \PassOptionsToPackage{numbers, compress}{natbib}
% % before loading neurips_2025


% % ready for submission
% \usepackage{neurips_2025}
% \usepackage{amsmath}
% \usepackage{graphicx}
% % to compile a preprint version, e.g., for submission to arXiv, add add the
% % [preprint] option:
% %     \usepackage[preprint]{neurips_2025}


% % to compile a camera-ready version, add the [final] option, e.g.:
% %     \usepackage[final]{neurips_2025}


% % to avoid loading the natbib package, add option nonatbib:
% %    \usepackage[nonatbib]{neurips_2025}


% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors


% \title{Graph-Based Operator Learning from Limited Data on Irregular Domains}


% % The \author macro works with any number of authors. There are two commands
% % used to separate the names and addresses of multiple authors: \And and \AND.
% %
% % Using \And between authors leaves it to LaTeX to determine where to break the
% % lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% % authors names on the first line, and the last on the second line, try using
% % \AND instead of \And before the third author name.


% \author{%
%   David S.~Hippocampus\thanks{Use footnote for providing further information
%     about author (webpage, alternative address)---\emph{not} for acknowledging
%     funding agencies.} \\
%   Department of Computer Science\\
%   Cranberry-Lemon University\\
%   Pittsburgh, PA 15213 \\
%   \texttt{hippo@cs.cranberry-lemon.edu} \\
%   % examples of more authors
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \AND
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
% }

% \begin{document}


% \maketitle


% \begin{abstract}
% Operator learning seeks to approximate mappings from input functions to output solutions, particularly in the context of partial differential equations (PDEs). While recent advances such as DeepONet and the Fourier Neural Operator (FNO) have demonstrated strong performance, they often rely on regular grid discretizations, limiting their applicability to complex or irregular domains. In this work, we propose a graph-based operator learning framework that addresses this limitation by constructing graphs from irregularly sampled spatial points and leveraging Graph Neural Networks (GNNs) to model spatial dependencies. To enhance representational power, we introduce a Fourier-based encoder that projects input functions into a frequency space using learnable complex coefficients, allowing for flexible embeddings even with sparse or nonuniform samples. We evaluated our approach across a range of 2D PDEs, including Darcy flow, Advection, Eikonal, and Non-linear Diffusion, under varying sampling densities. Our method consistently outperforms baselines, particularly in low-data regimes, demonstrating strong generalization and efficiency on irregular domains.


% \end{abstract}

% \section{Introduction}


% Learning mappings between function spaces is a fundamental task in computational physics and scientific machine learning, especially for approximating solution operators of partial differential equations (PDEs). Classical numerical solvers, such as finite element or finite difference methods, typically rely on mesh-based discretizations that can be restrictive or inefficient for complex geometries and irregular data. Operator learning offers a paradigm shift by learning the solution operator directly from data, enabling fast, mesh-free predictions across varying input conditions. As the demand grows for physics-informed machine learning models that are both data-efficient and generalizable to new regimes, operator learning has emerged as a powerful framework to bridge data-driven methods and physical laws, making it particularly relevant for real-time simulations, scientific discovery, and engineering design.
% Despite their success, existing operator learning models such as DeepONet \citep{lu2019deeponet} and Fourier Neural Operator (FNO) \citep{li2020fourier} exhibit notable limitations that restrict their applicability in more general settings. A key shortcoming lies in their reliance on regular, uniform grid discretizations—FNO, for instance, requires inputs to be defined on fixed Cartesian grids to leverage fast Fourier transforms efficiently. This assumption limits their flexibility and generalization ability when applied to problems defined on complex geometries, irregular meshes, or unstructured domains, which are common in real-world physical systems. Furthermore, these models often struggle with sparse or non-uniformly sampled data, leading to degraded performance and increased computational cost when adapting to more realistic, heterogeneous scenarios. Addressing these limitations is crucial for advancing operator learning towards broader scientific and engineering applications.


%  In contrast, Graph Kernel Network (GKN) \citep{li2020neural} introduces a powerful and efficient framework for learning operators that solve PDEs. By embedding PDE problems onto graph structures, GKN leverages graph kernel convolution layers to directly approximate continuous mappings between infinite-dimensional function spaces, enabling seamless generalization across varying discretizations, resolutions, and geometries.

% To address these limitations, we propose a graph-based operator learning framework that leverages Graph Neural Networks (GNNs) to learn PDE solution operators over irregular spatial domains. By constructing graphs from sampled spatial coordinates and encoding local geometric and functional dependencies through message passing, the model naturally adapts to non-Euclidean geometries. To enhance global expressivity, we further incorporate a Fourier-based encoder that projects input functions into a frequency domain using learnable complex-valued bases. This hybrid representation captures both global patterns and local interactions in a unified architecture.


% The contribution mainly lies in the following aspects:

% \begin{itemize}
%     \item  We evaluate our method across a variety of canonical PDEs including Darcy flow, Advection, Eikonal, and Non-linear Diffusion under varying data regimes and sampling densities. Our results demonstrate that the proposed approach consistently outperforms the baseline GKN in data-scarce settings and irregular domains, highlighting its potential for scalable and flexible operator learning.


% \end{itemize}









% % This adaptability makes them particularly well-suited for problems with unstructured meshes, varying resolution, or data collected from sensor networks and physical simulations in irregular geometries.


% % Moreover, by leveraging relational inductive biases and localized message passing, our method can better generalize across different domain shapes and resolutions, overcoming key limitations of grid-based methods like FNO and DeepONet.



% % Our model exhibits superior data efficiency and generalization, achieving lower prediction errors with fewer training samples and demonstrating robustness under domain shifts. By leveraging the structural flexibility of graphs and attention-based mechanisms, such models can capture fine-grained local interactions and long-range dependencies more effectively. As a result, graph-based architectures are emerging as a compelling direction for building data-driven solvers that are both physically grounded and practically deployable in complex scientific settings.



% \section{Related Work}




% % \section{Methodology}

% % \subsection{Problem Formulation}

% % Operator learning aims to approximate a mapping from input parameters and/or functions to their corresponding output functions. This framework is especially relevant in the context of solving partial differential equations (PDEs), where the goal is to learn the solution operator of a given PDE system.

% % Consider the following PDE:
% % \begin{equation}
% %     \mathcal{N}[u](\mathbf{x}) = f(\mathbf{x}), \quad \mathbf{x} \in \Omega \times [0, \infty),
% % \end{equation}
% % where $\mathbf{x}$ denotes a compact representation of the spatial and temporal coordinates, $\Omega$ is the spatial domain, and $[0, \infty)$ is the temporal domain. The operator $\mathcal{N}$ is a nonlinear differential operator, $u(\mathbf{x})$ is the unknown solution, and $f(\mathbf{x})$ is a given source term.

% % The objective is to learn the solution operator $\psi : \mathbb{F} \to \mathbb{U}$, where $\mathbb{F}$ and $\mathbb{U}$ are appropriate functional spaces. To do so, we use a training dataset
% % \[
% % \mathcal{D} = \{ (f_n, u_n) \}_{n=1}^N,
% % \]
% % comprising multiple input-output function pairs, where each $f_n(\cdot)$ and $u_n(\cdot)$ is discretized or sampled over a set of locations.


% % While early approaches such as DeepONet and the Fourier Neural Operator (FNO) have demonstrated promising results, they typically assume regular, grid-based discretizations of the domain. This assumption limits their applicability in settings with unstructured meshes, complex geometries, or adaptive sampling. To address this limitation, we leverage Graph Neural Networks for operator learning to model arbitrary domains via graph representations.

% % Once trained, the operator learning model can efficiently predict the solution $u$ for a new instance of the input $f$ at random locations.






% % \subsection{Graph Construction}
% % We first generate a grid of evenly spaced points in 2d space. Then we randomly selecte subset of these points. Based on these points, we construct graph by connecting points according to their spatial distance or probability. Here we need to define how to connect the sampled points into a graph, by creating an edge index that stores pairs of point indices. We connect points if they are within an Euclidean distance $r$. 
% % % We also build a probabilistic graph using a Gaussian kernel which aims to get edge probabilities and then randomly sample edges using these probabilities.
% % We define edge attributes including spatial coordinates and node features between source node and target node.









% % \subsection{Fourier Encoder}

% % We first design a fourier encoder to map $f$ values with their corresponding coordinates to an embedding by learning complex-valued fourier coefficients $\eta$.

% % Specifically, we compute fourier basis at the given coordinates using
% % \begin{align}
% %     \phi_k(x) = e^{2\pi i \langle x, \xi_k \rangle}
% % \end{align}
% % where $\xi_k$ is $k-th$ mode's frequency.

% % Then project to frequency space using an inner product with each frequency mode, 
% % \begin{align}
% %     f'_k = \frac{f \cdot \phi_k(x)^*}{N}
% % \end{align}
% % where $\phi_k(x)^*$ is conjugate of $\phi_k(x)$, $N$ is the number of points.



% % Then we transform $f$ in frequency space using learned complex weights $\eta$. 

% % \begin{align}
% %     g=f' \cdot \eta
% % \end{align}
% % where $f'$ is $[batch,channel,modes]$, $\eta$ is $[channel,dim,modes]$,
% % $g$ is $[batch,dim,modes]$.


% % Finally, we inverse projection to return to physical space using Fourier basis

% % \begin{align}
% %     h=g \cdot \phi(x)
% % \end{align}
% % where $\phi(x)$ is $[batch,N,modes]$, $h$ is $[batch,dim,N]$.

% % \subsection{Message Passing}


% %  $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ be a graph with nodes $i \in \mathcal{V}$, and edges $(i, j) \in \mathcal{E}$.
% % $h_i \in \mathbb{R}^{dim}$ be the feature vector of node $i$.
% % $\mathcal{N}(i)$ be the set of neighbors of node $i$.


% % For each edge $(j \to i) \in \mathcal{E}$,
% % \begin{align}
% %     h_{j \to i} = m(h_i, h_j, e_{j \to i})
% % \end{align}
% % where
% % $h_j$ is source node features,
% % $h_i$ is target node features,
% % $e_{j \to i}$ is edge features.

% % Each node $i$ aggregates the incoming messages
% % \begin{align}
% %     m_i = a \left( \left\{ h_{j \to i} \mid j \in \mathcal{N}(i) \right\} \right)
% % \end{align}

% % Each node updates its representation using the aggregated message
% % \begin{align}
% %     h'_i = u(h_i, m_i)
% % \end{align}

% % Then we concatenate $h$ and $h'$ and put it in linear layers.

% % The following is a three layers MLP with uniform initialization.

% % \textbf{Self-Attention}

% % We use linear layer to get query, key, value, and then calculate $h$ by

% % \begin{align}
% %     h= Q \cdot (K^T \cdot V) \cdot w
% % \end{align}
% % where $w$ is a uniform weights calculated by the number of points.
% % Then we use a linear layer to get the output.

% % \textbf{Graph Attention}

% % We take $h$ as input, and go through three linear layers to get $q,k,v$ correspondingly.

% % \begin{align}
% %     h_i' = \sum_{j \in \mathcal{N}(i)} \phi_m\left( q_i, k_j, v_j, e_{ij} \right)
% % \end{align}


% % \begin{align}
% %     \phi_m(q_i, k_j, v_j, e_{ij}) = \alpha_{ij} \cdot v_j
% % \end{align}

% % \begin{align}
% %     \alpha_{ij} = \frac{
% % \exp\left( \text{sim}(q_i, k_j, e_{ij}) \right)
% % }{
% % \sum_{k \in \mathcal{N}(i)} \exp\left( \text{sim}(q_i, k_k, e_{ik}) \right)
% % }
% % \end{align}


% % \begin{align}
% %     \text{sim}(q_i, k_j, e_{ij}) = \frac{
% % q_i^\top k_j + f(e_{ij})
% % }{\sqrt{d}}
% % \end{align}
% % where $f(\cdot)$ is a MLP.
% % Then we concatenate all heads' output, and add a residual part.
% % Finally, we go through a linear layer to get the predicted $u$.

% \section{Methodology}

% \subsection{Problem Formulation}

% Operator learning aims to approximate a mapping from input parameters and/or functions to their corresponding output functions. This framework is especially relevant in the context of solving partial differential equations (PDEs), where the goal is to learn the solution operator of a given PDE system.

% Consider the following PDE
% \begin{equation}
%     \mathcal{N}[u](\mathbf{x}) = f(\mathbf{x}), \quad \mathbf{x} \in \Omega \times [0, \infty),
% \end{equation}
% where $\mathbf{x}$ denotes a compact representation of the spatial and temporal coordinates, $\Omega$ is the spatial domain, and $[0, \infty)$ is the temporal domain. The operator $\mathcal{N}$ is a nonlinear differential operator, $u(\mathbf{x})$ is the unknown solution, and $f(\mathbf{x})$ is a given source term.

% The objective is to learn the solution operator $\psi : \mathbb{F} \to \mathbb{U}$, where $\mathbb{F}$ and $\mathbb{U}$ are appropriate functional spaces. To do so, we use a training dataset
% $\mathcal{D} = \{ (f_n, u_n) \}_{n=1}^N$,

% comprising multiple input-output function pairs, where each $f_n(\cdot)$ and $u_n(\cdot)$ is discretized or sampled over a set of locations.


% While early approaches such as DeepONet and the Fourier Neural Operator (FNO) have demonstrated promising results, they typically assume regular, grid-based discretizations of the domain. This assumption limits their applicability in settings with unstructured meshes, complex geometries, or adaptive sampling. To address this limitation, we leverage Graph Neural Networks for operator learning to model arbitrary domains via graph representations.

% Once trained, the operator learning model can efficiently predict the solution $u$ for a new instance of the input $f$ at random locations.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/model_flow.pdf}  % Adjust path and size
%     \caption{Work Flow}
%     \label{fig:my_pdf}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/model.pdf}  % Adjust path and size
%     \caption{Model}
% \end{figure}



% \subsection{Graph Construction}

% To represent PDE solutions over irregular domains, we begin by randomly sampling a subset of points $\{x_i\}^N_{i=1}$ from a uniform grid in 2D space. We then construct a graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ with nodes $\mathcal{V}=\{x_i\}$ and edges $\mathcal{E}$ determined by a radius $r$. Edges are created based on spatial proximity. Two nodes are connected if the Euclidean distance between them is less than a threshold $r$ such that 
% \begin{align}
%   (i,j) \in \mathcal{E} \quad \text{if and only if} \quad \| x_i - x_j \|_2 \leq r.  
% \end{align}




% Each edge $(i, j)$ carries edge attributes $e_{ij}$ that encode both geometric and feature-based information, such as the relative coordinates and function values at nodes $i$ and $j$ such that
% \begin{align}
% e_{ij} = \mathbin\Vert (x_i, x_j, f(x_i), f(x_j))
% \end{align}
% where $\mathbin\Vert$ is the concatenation operation.

% The adjacency matrix $A \in \mathbb{R}^{m \times m}$ is symmetrized and row-normalized as
% \begin{align}
%     \hat{A} = D^{-\frac{1}{2}} (A + I) D^{-\frac{1}{2}}
% \end{align}
% where $D$ is the degree matrix.


% This graph-based representation allows us to model unstructured spatial domains and enables message passing among nonuniform samples.


% \subsection{Fourier Encoder}


% We define a set of learnable frequencies
% \begin{align}
%    \left\{ \omega_m \in \mathbb{R}^2 \,\middle|\, m = 1, \ldots, M \right\} 
% \end{align}

% For any coordinate $ x \in \mathbb{R}^2 $, the $m$-th basis function is given by the complex exponential
% \begin{align}
%     \varphi_m(x) = e^{2\pi i \langle \omega_m, x \rangle}
% \end{align}

% where $\langle \cdot, \cdot \rangle$ denotes the standard Euclidean inner product, and $i$ is the imaginary unit.


% At the discrete level, for a batch of $B$ samples and $N$ points per sample, the basis matrix is defined as
% \begin{align}
%     \Phi \in \mathbb{C}^{B \times N \times M}, \quad \Phi_{b,i,m} = e^{2\pi i \langle \omega_m, x_i^{(b)} \rangle}.
% \end{align}
% where $x_i^{(b)}$ denotes the $i$-th coordinate point in the $b$-th batch sample.


% Given the input $f \in \mathbb{R}^{B \times C_{\text{in}} \times N}$ sampled at points $\{ x_i \}$, we first project onto the Fourier basis.

% We compute the Fourier coefficients by
% \begin{align}
%     \hat{u}_{b,c,m} = \frac{1}{N} \sum_{i=1}^{N} f_{b,c,i} \, \overline{\varphi_m\left(x_i^{(b)}\right)}
% \end{align}
% where $\overline{(\cdot)}$ denotes complex conjugation.

% We introduce a learnable set of complex Fourier coefficients as
% \begin{align}
%    W \in \mathbb{C}^{C_{\text{in}} \times C_{\text{out}} \times M}
% \end{align}

% The spectral filtering operation is
% \begin{align}
%     \hat{v}_{b,o,m} = \sum_{c=1}^{C_{\text{in}}} \hat{u}_{b,c,m} \, W_{c,o,m}.
% \end{align}


% We reconstruct the output in the physical domain by applying the inverse transform
% \begin{align}
%     v_{b,o,i} = \sum_{m=1}^{M} \hat{v}_{b,o,m} \, \varphi_m\left(x_i^{(b)}\right).
% \end{align}


% Since $v$ is complex-valued, we only take its real part for the output as
% \begin{align}
%     h = \text{Re}(v) \in \mathbb{R}^{B \times C_{\text{out}} \times N}
% \end{align}


% This step captures global interactions over the irregular domain.
% The output $h$ serves as the input node features for the downstream GNN model.



% \subsection{Message Passing}

% Given a node $i \in \mathcal{V}$ and its set of neighbors $\mathcal{N}(i)$, the pre-processed messages $\{ m_{ij} \}_{j \in \mathcal{N}(i)}$ are first computed using a learnable neural network $g_{\Theta}$ as
% \begin{align}
%   m_{ij} = g_{\Theta}(h_i, h_j, e_{ij})  
% \end{align}
% where $h_i$ and $h_j$ are node features, and $e_{ij}$ denotes edge attributes.

% Then we aggregate message from neighbors such that
% \begin{align}
%     \hat{m} = \mathbin\Vert (\frac{1}{|\mathcal{N}(i)|} \sum_{j \in \mathcal{N}(i)} m_{ij}, \max_{j \in \mathcal{N}(i)} m_{ij}, \min_{j \in \mathcal{N}(i)} m_{ij},  \sqrt{ \frac{1}{|\mathcal{N}(i)|} \sum_{j \in \mathcal{N}(i)} (m_{ij} - \frac{1}{|\mathcal{N}(i)|} \sum_{j \in \mathcal{N}(i)} m_{ij})^2 })
% \end{align}


% This concatenated feature vector is processed by a post-aggregation neural network \( \gamma_{\Theta} \) to produce the updated node representation by
% \begin{align}
%   h_i' = \gamma_{\Theta}\left( h_i, \hat{m} \right)
% \end{align}
% The updated node representation is passed through additional MLP layers with residual connections to enhance expressiveness.

% \subsection{Multi-Head Self-Attention}


% We employ $H$ independent attention heads. For each head $h$,
% the query, key and value functions are computed as linear projections
% \begin{align}
% q^{(h)}(x) = W_q h'(x), \quad
% k^{(h)}(y) = W_k h'(y), \quad
% v^{(h)}(y) = W_v h'(y)
% \end{align}
% where $W_q, W_k, W_v \in \mathbb{R}^{d_h \times C_{\text{out}}}$, $q^{(h)}(x), k^{(h)}(y), v^{(h)}(y) \in \mathbb{R}^{d_h}$ are learned head-specific features, and $d_h$ is the dimension per attention head.

% Before computing attention, the keys and values are normalized
% \begin{align}
% \tilde{k}^{(h)}(y) = \text{Norm}(k^{(h)}(y)), \quad
% \tilde{v}^{(h)}(y) = \text{Norm}(v^{(h)}(y)),
% \end{align}
% where $\text{Norm}(\cdot)$ denotes instance normalization.

% We first compute
% \begin{align}
% G_h = \sum_{j=1}^N k^{(h)}(y_j)^\top v^{(h)}(y_j) w(y_j)
% \end{align}
% where $G_h \in \mathbb{R}^{d_h \times d_h}$, $w$ is calculated by the number of points,
% and then
% \begin{align}
% (\mathcal{K}_h h')(x_i) = q^{(h)}(x_i) G_h.
% \end{align}


% The outputs are concatenated as
% % \begin{align}
% %   (\mathcal{K}h')(x_i) = \text{concat}\left( (\mathcal{K}_1 h')(x_i), \ldots, (\mathcal{K}_H h')(x_i) \right)  
% % \end{align}

% \begin{align}
%   (\mathcal{K}h')(x_i) = \mathbin\Vert \left( (\mathcal{K}_1 h')(x_i), \ldots, (\mathcal{K}_H h')(x_i) \right)  
% \end{align}





% and projected to the output space by
% \begin{align}
% \hat{h}(x_i) = W_{\text{out}} (\mathcal{K}h')(x_i)
% \end{align}
% where $W_{\text{out}} \in \mathbb{R}^{C_{\text{out}} \times (C_{\text{out}} \cdot H)}$.

% The result is then passed through a linear projection layer to update the node features.



% \subsection{Message Passing with Attention}


% The attention weights $\alpha_{ij}$ are computed using a scaled dot-product attention mechanism by
% \begin{align}
%     \alpha_{ij} = \text{softmax}_j \left( \frac{ \left( W_4 \hat{h}_i \right)^\top \left( W_5 \hat{h}_j + W_3 e_{ij} \right) }{ \sqrt{d} } \right),
% \end{align}
% where $d$ is the dimensionality of the head, and the softmax is applied over the set of neighbors $j \in \mathcal{N}(i)$.

% Then we update node features using
% \begin{align}
%   \hat{h}_i' = W_1 \hat{h}_i + \sum_{j \in \mathcal{N}(i)} \alpha_{ij} \left( W_2 \hat{h}_j + W_3 e_{ij} \right)  
% \end{align}



% A skip connection is introduced
% \begin{align}
%     \hat{h}_i' = \hat{h}_i' + W_s \hat{h}_i
% \end{align}
% where $W_s$ is a learnable weight matrix.
% Then we add a linear projection to produce the predicted solution $\hat{u}$.


% \subsection{Training}

% The model is trained to minimize the relative $L_2$ error between predicted and true solutions

% \begin{align}
%     \mathcal{L}(\theta) = \frac{ \| u - \psi_\theta(f) \|_{L^2(\Omega)} }{ \| u \|_{L^2(\Omega)} }
% \end{align}



% \section{Experiments}

% We tested on four 2D PDE datasets including Darcy Flow, Nonlinear Diffusion, Eikonal, Poisson.


% For each dataset we simulated $Ntrain \in \{5,10,20,30,40,50,80,100\}$
% examples for training, 100 examples for testing.

% We randomly sampled $N \in \{20,30,40,50,60,70,80,90,100, 200, 300, 400, 500, 600, 700,800,\\ 900,1000\}$ points on a uniform $128 \times 128$ grid on the domain $[0,1] \times [0,1]$ 
%  to construct a graph.

% The sampled points serve as the nodes of the graph. The model is then trained to approximate the underlying solution operator based on these irregularly sampled data.

% \subsection{Results}

% Baselines include DeepONet, Fourier Neural Operator (FNO), Graph Convolutional Network(GCN), Graph Kernel Network(GKN).

% We tested DeepONet, FNO, GCN on $128 \times 128$ grid data, and tested GKN and our model on 4000 sample data randomly selected from $128 \times 128$ grid data. We used training data size $\in \{5,10,20,30,40,50,80,100\}$ to test in these five models on four PDE benchmarks. Our test data size was 100. We can conclude that our model performed much better than GKN in all cases.






% % \begin{table*}[h]
% % % \caption{\small training data size is 100, test data size is 100, sample points is 200 }
% %     \small
% %     \centering


% %     \begin{subtable}{\textwidth}
% %     \caption{\small \textit{training data size is 5}}
% %     \small 
% %     \centering
% % \begin{tabular}{cccc}
% %     \hline
% %     \textit{Dataset}      &  & GCN   & DeepONet  & FNO    & GKN            \\ \hline
% %     Darcy Flow                  &  & 2.3658	& 1.1285 & 0.4458 & 0.4458      \\ \hline
% %     Advection   &  & 1.0137	& 0.8814  & 0.8845  & 0.4458   \\ \hline
% %     Eikonal            &  & 0.2284     & 0.2305 & 4.7221 & 0.4458 \\ \hline
% %     Nonlinear Diffusion            &  & 0.3012    & 0.3720 & 0.2580  & 0.4458\\ \hline
% %      \hline
% % \end{tabular}
% % \end{subtable}  

% % \end{table*}

% \begin{table*}[h]
%     \centering
%     \small
%     % \begin{subtable}{\textwidth}
%     %     \caption{\small \textit{Test errors for different models trained on 5 training data size across various PDE benchmarks.}}
%     %     \centering
%     %     \begin{tabular}{lccccc}
%     %         \toprule
%     %         \textit{Dataset} & GCN & DeepONet & FNO & GKN & Ours \\
%     %         \midrule
%     %         Darcy Flow           & 2.3658 & 1.1285 & 0.4458 & 0.4080 & \textbf{0.4795} \\
%     %         Advection            & 1.0137 & 0.8814 & 0.8845 & 1.0576 & 0.7151\\
%     %         Eikonal              & 0.2284 & 0.2305 & 4.7221 & 0.1979 & 0.1599 \\
%     %         Nonlinear Diffusion & 0.3012 & 0.3720 & 0.2580 & 0.2831 & 0.1570 \\
%     %         \bottomrule
%     %     \end{tabular}
%     % \end{subtable}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test errors for different models trained on 10 training data size across various PDE benchmarks.}}
%         \centering
%         \begin{tabular}{lccccc}
%             \toprule
%             \textit{Dataset} & GCN & DeepONet & FNO & GKN & Ours\\
%             \midrule
%             Darcy Flow           & 2.3676 & 0.9993 & 0.3185 & 0.3345 & \text{0.2787} \\
%             Advection            & 1.0093 & 0.5988 & 0.6353 & 1.0026 & 0.6668\\
%             Eikonal              & 0.2190 & 0.2029 & 0.1539 & 0.1956 & \text{0.1286} \\
%             Nonlinear Diffusion & 0.2774 & 0.3307 & 0.1355 & 0.2346 & \text{0.1204} \\
%             \bottomrule
%         \end{tabular}
%     \end{subtable}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test errors for different models trained on 20 training data size across various PDE benchmarks.}}

%         \centering
%         \begin{tabular}{lccccc}
%             \toprule
%             \textit{Dataset} & GCN & DeepONet & FNO & GKN & Ours\\
%             \midrule
%             Darcy Flow           & 0.9697 & 0.5768 & 0.2345 & 0.2660 & 0.2005 \\
%             Advection            & 0.9943 & 0.3727 & 0.4243 & 0.7421 & 0.4790\\
%             Eikonal              & 0.2149 & 0.1559 & 0.1175 & 0.1697 & 0.1059 \\
%             Nonlinear Diffusion & 0.2664 & 0.2713 & 0.1031 & 0.1716 & 0.0599 \\
%             \bottomrule
%         \end{tabular}
%     \end{subtable}




%     \small
%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test errors for different models trained on 30 training data size across various PDE benchmarks.}}
%         \centering
%         % \caption{\small \textit{Training data size is 30}}
%         \begin{tabular}{lccccc}
%             \toprule
%             \textit{Dataset} & GCN & DeepONet & FNO & GKN & Ours \\
%             \midrule
%             Darcy Flow            & 1.3902 & 0.4163 & 0.1678 & 0.2375 & 0.1554 \\
%             Advection             & 0.9620 & 0.3925 & 0.3873 & 0.5353 & 0.3707 \\
%             Eikonal               & 0.2120 & 0.1442 & 0.0874 & 0.1530 & 0.0803 \\
%             Nonlinear Diffusion   & 0.2703 & 0.2468 & 0.0793 & 0.1520 & 0.0747 \\
%             \bottomrule
%         \end{tabular}
%     \end{subtable}

    

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test errors for different models trained on 40 training data size across various PDE benchmarks.}}
%         \centering
%         \begin{tabular}{lccccc}
%             \toprule
%             \textit{Dataset} & GCN & DeepONet & FNO & GKN & Ours\\
%             \midrule
%             Darcy Flow           & 0.9599 & 0.3387 & 0.1426 & 0.1994 & 0.1112 \\
%             Advection            & 0.9611 & 0.3331 & 0.3303 & 0.4570 & 0.3381\\
%             Eikonal              & 0.2063 & 0.1502 & 0.0699 & 0.1306 & 0.0875 \\
%             Nonlinear Diffusion & 0.2613 & 0.2117 & 0.0490 & 0.1425 & 0.0400 \\
%             \bottomrule
%         \end{tabular}
%     \end{subtable}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test errors for different models trained on 50 training data size across various PDE benchmarks.}}
%         \centering
%         \begin{tabular}{lccccc}
%             \toprule
%             \textit{Dataset} & GCN & DeepONet & FNO & GKN & Ours\\
%             \midrule
%             Darcy Flow           & 0.8930 & 0.3162 & 0.1200 & 0.1890 & 0.1597 \\
%             Advection            & 0.9543 & 0.2394 & 0.2716 & 0.3717 & 0.3550\\
%             Eikonal              & 0.1935 & 0.1789 & 0.0642 & 0.1273 & 0.0895 \\
%             Nonlinear Diffusion & 0.2626 & 0.2195 & 0.0377 & 0.1218 & 0.0532 \\
%             \bottomrule
%         \end{tabular}
%     \end{subtable}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test errors for different models trained on 100 training data size across various PDE benchmarks.}}
%         \centering
%         \begin{tabular}{lccccc}
%             \toprule
%             \textit{Dataset} & GCN & DeepONet & FNO & GKN & Ours\\
%             \midrule
%             Darcy Flow           & 0.6378 & 0.2289 & 0.0645 & 0.1748 & 0.0741 \\
%             Advection            & 0.9575 & 0.1691 & 0.1847 & 0.2886 & 0.1952\\
%             Eikonal              & 0.1850 & 0.2052 & 0.0523 & 0.1168 & 0.0643 \\
%             Nonlinear Diffusion & 0.2474 & 0.1912 & 0.0223 & 0.1044 & 0.0302 \\
%             \bottomrule
%         \end{tabular}
%     \end{subtable}



    
    
% \end{table*}




% % \subsection{Generalization to New Resolutions}

% % Use point clouds with low, medium, and high sampling densities.yes

% % Fewer Points in Train, More in Test (Resolution Generalization Test): if the model trained on coarse/sparse data generalizes to denser evaluation since operator learning should ideally recover continuous mappings.
% % Train with 1000 points, test with 1000, 3000, 5000 points.


% % Train with 1000 points, test with 100 or 5000 points.

% % Train on low-res samples, test on high-res samples.

% \begin{table*}
%         \centering
%     \caption{\small \textit{Test errors with low, medium, and high test sampling densities with training data size=100}}
%     \small
%     \begin{tabular}{lccc}
%         \toprule
%         \text{\textit{Sample Density}} & \text{20} & \text{500} & \text{1000} \\
%         \midrule
%         Darcy Flow       & 0.4269 & 0.1433 & 0.1147 \\
%         Advection  & 0.3980 & 0.2462 & 0.2350 \\
%         Eikonal         & 0.1236 & 0.0671 & 0.0643 \\
%         Nonlinear Diffusion  & 0.2030 & 0.0637 & 0.0439 \\
%         \bottomrule
%     \end{tabular}
% \end{table*}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/Test_errors_sampling_densities.jpg}
%   \caption{Test errors with low, medium, and high sampling densities with training data size=100}
% \end{figure}


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/Test_errors_test_sampling_densities.jpg}
%   \caption{Test errors with low, medium, and high test sampling densities with training data size=100, train sampling density=1000}
% \end{figure}



% \begin{table}[ht]
%     \centering
%     \caption{\small \textit{Test errors with low, medium, and high test sampling densities with training sample points=1000, training data size=100}}
%     \label{tab:Ntr100_train1000_vary_test_pts}
%     \begin{tabular}{lccccc}
%         \toprule
%         % \textit{Dataset}      & \multicolumn{4}{c}{Test Sample Points} \\
%         % \cmidrule(lr){2-5}
%         \text{\textit{Test Sample Density}}                      & 100     & 500     & 1000    & 2000 & 4000    \\
%         \midrule
%         Darcy Flow            & 0.2419  & 0.1304  & 0.1147  & 0.0990  & 0.0913  \\
%         Advection             & 0.3757  & 0.2535  & 0.2350  & 0.2239  & 0.2181  \\
%         Eikonal               & 0.0819  & 0.0687  & 0.0643  & 0.0610  & 0.0604  \\
%         Nonlinear Diffusion   & 0.0945  & 0.0501  & 0.0495  & 0.0417  & 0.0415  \\
%         \bottomrule
%     \end{tabular}
% \end{table}


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/train_points1000_with_test.jpg}
%   \caption{Test error trend with training sampling density=1000}
% \end{figure}







% \begin{table*}
%         \centering
%     \caption{ \small \textit{Test error for each PDE evaluated under varying numbers of training data size with sample density=4000} }
%     \small
%     \begin{tabular}{lccccc}
%         \toprule
%         % \multicolumn{6}{c}{\textit{sample density} = 4000} \\
%         % \midrule
%         \textit{Training data size} & 20     & 40     & 60     & 80     & 100    \\
%         \midrule
%         Darcy Flow        & 0.2005 & 0.1112 & 0.0905 & 0.0863 & 0.0724 \\
%         Advection    & 0.4790 & 0.3381 & 0.3184 & 0.2380 & 0.1952 \\
%         Eikonal          & 0.1112 & 0.0934 & 0.0762 & 0.0673 & 0.0667 \\
%         Nonlinear Diffusion    & 0.0599 & 0.0400 & 0.0342 & 0.0312 & 0.0302 \\
%         \bottomrule
%     \end{tabular}



% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=900}}
%         \centering

%     \begin{tabular}{lcccccccc}
%         \toprule
%         % \multicolumn{8}{c}{Test sample points = 900} \\
%         % \midrule
%         \textit{Training data size} & 5      & 10     & 20     & 30     & 40     & 50    & 80   & 100    \\
%         \midrule
%         Darcy Flow      & 0.4996 & 0.2812 & 0.2215 & 0.1587 & 0.1503 & 0.1360 & 0.1230 & 0.1168\\
%         Advection  & 0.6921 & 0.6862 & 0.4866 & 0.4074 & 0.3560 & 0.3460 & 0.2601 & 0.2310 \\
%         Eikonal         & 0.1540 & 0.1245 & 0.1059 & 0.0760 & 0.0718 & 0.0704 & 0.0694 & 0.0655\\
%         Nonlinear Diffusion  & 0.1589 & 0.1420 & 0.0740 & 0.0683 & 0.0595 & 0.0567 & 0.0474 & 0.0463\\
%         \bottomrule
%     \end{tabular}

% \end{subtable}


% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=800}}
%         \centering

%   \begin{tabular}{lcccccccc}
%     \toprule
%     \textit{Training data size} & 5      & 10     & 20     & 30     & 40     & 50     & 80     & 100    \\
%     \midrule
%     Darcy Flow      & 0.5102 & 0.2781 & 0.2303 & 0.1576 & 0.1572 & 0.1381 & 0.1243 & 0.1226 \\
%     Advection   & 0.7407 & 0.7109 & 0.4799 & 0.4148 & 0.3789 & 0.3641 & 0.2791 & 0.2408 \\
%     Eikonal         & 0.1606 & 0.1210 & 0.1038 & 0.0756 & 0.0731 & 0.0730 & 0.0697 & 0.0625 \\
%     Nonlinear Diffusion  & 0.1623 & 0.1406 & 0.0728 & 0.0706 & 0.0701 & 0.0652 & 0.0501 & 0.0469 \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}



% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=700}}
%         \centering

%   \begin{tabular}{lcccccccc}
%     \toprule
%     \textit{Training data size} & 5      & 10     & 20     & 30                           & 40     & 50                           & 80                           & 100    \\
%     \midrule
%     Darcy Flow           & 0.4985 & 0.2768 & 0.2332 & 0.1659 & 0.1592 & 0.1506 & 0.1301 & 0.1235 \\
%     Advection            & 0.6978 & 0.6590 & 0.5594 & 0.4172 & 0.3747 & 0.3364 & 0.2926 & 0.2421 \\
%     Eikonal              & 0.1605 & 0.1180 & 0.1038 & 0.0801 & 0.0755 & 0.0713 & 0.0643 & 0.0635 \\
%     Nonlinear Diffusion  & 0.1642 & 0.1363 & 0.0731 & 0.0696 & 0.0623 & 0.0575 & 0.0548       & 0.0507 \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}

% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=600}}
%         \centering

%   \begin{tabular}{lcccccccc}
%     \toprule
%     \textit{Training data size}
%     % \multicolumn{1}{l}{\textit{Training data size}} 
%       & 5      & 10     & 20     & 30     & 40     & 50  & 80   & 100    \\
%     % \cmidrule(l){1-1}
%     \midrule
    
%     Darcy Flow          & 0.4817 & 0.2886 & 0.2362 & 0.1646 & 0.1616 & 0.1497 & 0.1401 & 0.1376 \\
%     Advection           & 0.7537 & 0.7271 & 0.5754 & 0.4109 & 0.3661 & 0.3378 & 0.3216 & 0.2453 \\
%     Eikonal             & 0.1483 & 0.1255 & 0.1073 & 0.0776 & 0.0772 & 0.0745 & 0.0691 & 0.0665 \\
%     Nonlinear Diffusion & 0.2149 & 0.1440 & 0.0781 & 0.0709 & 0.0644 & 0.0618 & 0.0583 & 0.0553 \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}


% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=500}}
%         \centering

% \begin{tabular}{lcccccccc}
% \toprule
% \textit{Training data size} & 5     & 10    & 20    & 30    & 40    & 50    & 80 & 100   \\
% \midrule
% Darcy Flow             & 0.4855 & 0.2842 & 0.2247 & 0.1772 & 0.1643 & 0.1609 & 0.1414 & 0.1315 \\
% Advection              & 0.7947 & 0.7011 & 0.5431 & 0.4089 & 0.3609 & 0.3468 & 0.3299 & 0.2462 \\
% Eikonal                & 0.1537 & 0.1155 & 0.1060 & 0.0901 & 0.0811 & 0.0702 & 0.0689 & 0.0671 \\
% Nonlinear Diffusion    & 0.1686 & 0.1464 & 0.0801 & 0.0773 & 0.0760 & 0.0733 & 0.0626 & 0.0594 \\
% \bottomrule
% \end{tabular}

% \end{subtable}

% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=400}}
%         \centering

% \begin{tabular}{lcccccccc}
% \toprule
% \textit{Training data size} & 5      & 10     & 20     & 30     & 40     & 50  & 80   & 100    \\
% \midrule
% Darcy Flow           & 0.4970 & 0.3109 & 0.2471 & 0.1864 & 0.1804 & 0.1741 & 0.1481 & 0.1415 \\
% Advection            & 0.7604 & 0.6733 & 0.5317 & 0.4090 & 0.4005 & 0.3658 & 0.3499 & 0.2516 \\
% Eikonal              & 0.1547 & 0.1203 & 0.1058 & 0.0908 & 0.0883 & 0.0829 & 0.0725 & 0.0669 \\
% Nonlinear Diffusion  & 0.1695 & 0.1411 & 0.0847 & 0.0815 & 0.0776 & 0.0766 & 0.0637 & 0.0618 \\
% \bottomrule
% \end{tabular}

% \end{subtable}


% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=300}}
%         \centering

% \begin{tabular}{lcccccccc}
% \toprule
% \textit{Training data size} & 5      & 10     & 20     & 30     & 40     & 50   & 80   & 100    \\
% \midrule
% Darcy Flow           & 0.5075 & 0.3233 & 0.2416 & 0.1906 & 0.1880 & 0.1771 & 0.1592 & 0.1479 \\
% Advection            & 0.7606 & 0.6674 & 0.5323 & 0.4191 & 0.4178 & 0.3882 & 0.3505 & 0.2537 \\
% Eikonal              & 0.1533 & 0.1246 & 0.1066 & 0.0921 & 0.0835 & 0.0824 & 0.0709 & 0.0664 \\
% Nonlinear Diffusion  & 0.1722 & 0.1498 & 0.0920 & 0.0873 & 0.0849 & 0.0818 & 0.0694 & 0.0674 \\
% \bottomrule
% \end{tabular}

% \end{subtable}


% \end{table*}

% \begin{table*}
    

% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=200}}
%         \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \textit{Training data size} & 5      & 10     & 20     & 30     & 40     & 50        &80              & 100    \\
% \midrule
% Darcy Flow           & 0.5227 & 0.3431 & 0.2812 & 0.2275 & 0.2222 & 0.2182                  & 0.1880 & 0.1878 \\
% Advection            & 0.7586 & 0.6407 & 0.5004 & 0.4123 & 0.4040 & 0.3931      & 0.3697 & 0.2880 \\
% Eikonal              & 0.1538 & 0.1276 & 0.1069 & 0.0981 & 0.0934 & 0.0873                  & 0.0780 & 0.0745 \\
% Nonlinear Diffusion  & 0.1807 & 0.1605 & 0.1060 & 0.1024 & 0.0951 & 0.0932                  & 0.0804 & 0.0755 \\
% \bottomrule
% \end{tabular}

% \end{subtable}

% % \end{table*}

% % \begin{table*}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=100}}
%         \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \textit{Training data size} &5 & 10     & 20     & 30     & 40     & 50   &80  & 100    \\
% \midrule
% Darcy Flow           & 0.5534 & 0.4673 & 0.3986 & 0.3705 & 0.2994 & 0.2918 & 0.2471 & 0.2349 \\
% Advection            & 0.7513 & 0.6738 & 0.5498 & 0.4977 & 0.4547 & 0.4130 & 0.4069 & 0.3216 \\
% Eikonal              & 0.1583 & 0.1402 & 0.1115 & 0.1047 & 0.1044 & 0.0988 & 0.0876 & 0.0857 \\
% Nonlinear Diffusion  & 0.2062 & 0.1691 & 0.1332 & 0.1234 & 0.1161 & 0.1157 & 0.0995 & 0.0947 \\
% \bottomrule
% \end{tabular}

% \end{subtable}

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=90}}
%         \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \textit{Training data size} & 5      & 10     & 20     & 30     & 40     & 50   & 80  & 100    \\
% \midrule
% Darcy Flow           & 0.6094 & 0.4362 & 0.3638 & 0.3225 & 0.2791 & 0.2785 & 0.2471 & 0.2420 \\
% Advection            & 0.6764 & 0.6612 & 0.5334 & 0.4470 & 0.4452 & 0.4238 & 0.3977 & 0.3315 \\
% Eikonal              & 0.1612 & 0.1401 & 0.1140 & 0.1088 & 0.1084 & 0.1083 & 0.0893 & 0.0891 \\
% Nonlinear Diffusion  & 0.2036 & 0.1693 & 0.1329 & 0.1279 & 0.1179 & 0.1110 & 0.1046 & 0.0995 \\
% \bottomrule
% \end{tabular}

% \end{subtable}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=80}}
%         \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \textit{Training data size} & 5      & 10     & 20     & 30     & 40     & 50   & 80  & 100    \\
% \midrule
% Darcy Flow           & 0.6076 & 0.4561 & 0.3709 & 0.3394 & 0.2994 & 0.2970 & 0.2633 & 0.2566 \\
% Advection            & 0.6579 & 0.6365 & 0.5318 & 0.4460 & 0.4450 & 0.4397 & 0.4049 & 0.3368 \\
% Eikonal              & 0.1561 & 0.1412 & 0.1170 & 0.1115 & 0.1113 & 0.1078 & 0.0937 & 0.0911 \\
% Nonlinear Diffusion  & 0.2086 & 0.1777 & 0.1401 & 0.1295 & 0.1225 & 0.1177 & 0.1116 & 0.1067 \\
% \bottomrule
% \end{tabular}

% \end{subtable}



%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=70}}
%         \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \textit{Training data size} & 5      & 10     & 20     & 30     & 40     & 50   & 80  & 100    \\
% \midrule
% Darcy Flow           & 0.6176 & 0.4682 & 0.3965 & 0.3565 & 0.3176 & 0.3151 & 0.2773 & 0.2864 \\
% Advection            & 0.6697 & 0.6654 & 0.5524 & 0.4583 & 0.4479 & 0.4400 & 0.4156 & 0.3626 \\
% Eikonal              & 0.1606 & 0.1450 & 0.1154 & 0.1138 & 0.1128 & 0.1121 & 0.1005 & 0.0953 \\
% Nonlinear Diffusion  & 0.2279 & 0.1776 & 0.1498 & 0.1369 & 0.1294 & 0.1285 & 0.1223 & 0.1206 \\
% \bottomrule
% \end{tabular}

% \end{subtable}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=60}}
%         \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \textit{Training data size} & 5      & 10     & 20     & 30     & 40                     & 50         & 80            & 100    \\
% \midrule
% Darcy Flow           & 0.5989 & 0.4762 & 0.4251 & 0.3733 & 0.3308                 & 0.2884                 & 0.2842 & 0.2711 \\
% Advection            & 0.6906 & 0.6342 & 0.5541 & 0.4537 & 0.4270                 & 0.4238                 & 0.4131 & 0.3662 \\
% Eikonal              & 0.1637 & 0.1483 & 0.1192 & 0.1162 & 0.1058   & 0.1052   & 0.1015 & 0.1020  \\
% Nonlinear Diffusion  & 0.2211 & 0.1963 & 0.1580 & 0.1408 & 0.1318                 & 0.1303                 & 0.1286 & 0.1248 \\
% \bottomrule
% \end{tabular}

% \end{subtable}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=50}}
%         \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \textit{Training data size} & 5      & 10     & 20     & 30     & 40                     & 50     & 80                & 100    \\
% \midrule
% Darcy Flow           & 0.6595 & 0.4944 & 0.4445 & 0.3902 & 0.3546                 & 0.3536                 & 0.3158 & 0.3072 \\
% Advection            & 0.6784 & 0.6219 & 0.5618 & 0.4580 & 0.4412                 & 0.4334                 & 0.4069 & 0.3747 \\
% Eikonal              & 0.1576 & 0.1498 & 0.1191 & 0.1174 & 0.1111   & 0.1103   & 0.1038 & 0.0981 \\
% Nonlinear Diffusion  & 0.2458 & 0.2048 & 0.1661 & 0.1523 & 0.1439                 & 0.1437                 & 0.1382 & 0.1369 \\
% \bottomrule
% \end{tabular}

% \end{subtable}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=40}}
%         \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \textit{Training data size} & 5      & 10     & 20     & 30     & 40     & 50 & 80    & 100    \\
% \midrule
% Darcy Flow           & 0.6693 & 0.5169 & 0.4674 & 0.4190 & 0.3840 & 0.3722 &0.3339 & 0.3328 \\
% Advection            & 0.6966 & 0.6941 & 0.5189 & 0.4642 & 0.4625 & 0.4361 &0.3901 & 0.3773 \\
% Eikonal              & 0.1712 & 0.1521 & 0.1255 & 0.1200 & 0.1172 & 0.1162 &0.1038 & 0.1060 \\
% Nonlinear Diffusion  & 0.2720 & 0.2439 & 0.1755 & 0.1647 & 0.1563 & 0.1485 &0.1500 & 0.1446 \\
% \bottomrule
% \end{tabular}

% \end{subtable}


% \end{table*}


% \begin{table*}
    

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=30}}
%         \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \textit{Training data size} & 5      & 10     & 20     & 30     & 40     & 50  & 80   & 100    \\
% \midrule
% Darcy Flow           & 0.7064 & 0.5529 & 0.5131 & 0.4509 & 0.4114 & 0.4064 & 0.3697 & 0.3663 \\
% Advection            & 0.7536 & 0.6746 & 0.4973 & 0.4655 & 0.4256 & 0.4046 & 0.3996 & 0.3883 \\
% Eikonal              & 0.1822 & 0.1606 & 0.1377 & 0.1313 & 0.1232 & 0.1213 & 0.1140 & 0.1125 \\
% Nonlinear Diffusion  & 0.3148 & 0.2735 & 0.2003 & 0.1878 & 0.1867 & 0.1858 & 0.1812 & 0.1795 \\
% \bottomrule
% \end{tabular}

% \end{subtable}

% % \end{table*}

% % \begin{table*}
%        \begin{subtable}{\textwidth}
%         \caption{\small \textit{Test sample density=20}}
%         \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \textit{Training data size} &5 & 10     & 20     & 30     & 40     & 50  & 80   & 100    \\
% \midrule
% Darcy Flow           & 0.7416& 0.5963 & 0.5363 & 0.4984 & 0.4567 & 0.4484 & 0.4176 & 0.4073 \\
% Advection            & 0.8587 & 0.7329 & 0.5114 & 0.4798 & 0.4661 & 0.4338 & 0.4186 & 0.3980 \\
% Eikonal              & 0.1875 & 0.1797 & 0.1543 & 0.1402 & 0.1392 & 0.1361 & 0.1292 & 0.1236 \\
% Nonlinear Diffusion  & 0.3202 & 0.3074 & 0.2403 & 0.2365 & 0.2297 & 0.2202 & 0.2000 & 0.1958 \\
% \bottomrule
% \end{tabular}

% \end{subtable}


% % \end{table*}











% % \begin{table*}

% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sampel density=100, train data size=100}}
%         \centering

%     \label{tab:Ntr100_Nte100_pts100}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.3402   & 0.2349  & 30.95\% \\
%         Advection             & 0.3446   & 0.3216  & 6.67\%  \\
%         Eikonal               & 0.1442   & 0.0857  & 40.57\% \\
%         Nonlinear Diffusion   & 0.1689   & 0.0947  & 43.93\% \\
%         \bottomrule
%     \end{tabular}

% \end{subtable}


% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=200, train data size=100}}
%         \centering

%     \label{tab:Ntr100_Nte100_pts200}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}          & GKN     & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow                & 0.2633  & 0.1878  & 28.67\% \\
%         Advection                 & 0.3150  & 0.2880  & 8.57\%  \\
%         Eikonal                   & 0.1325  & 0.0745  & 43.77\% \\
%         Nonlinear Diffusion       & 0.1415  & 0.0755  & 46.64\% \\
%         \bottomrule
%     \end{tabular}

% \end{subtable}

% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=300, train data size=100}}
%         \centering

%     \label{tab:Ntr100_Nte100_pts300}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.2355   & 0.1479  & 37.20\% \\
%         Advection             & 0.3017   & 0.2537  & 15.91\% \\
%         Eikonal               & 0.1238   & 0.0664  & 46.37\% \\
%         Nonlinear Diffusion   & 0.1245   & 0.0674  & 45.86\% \\
%         \bottomrule
%     \end{tabular}

% \end{subtable}



% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=400, train data size=100}}
%         \centering

%     \label{tab:Ntr100_Nte100_pts400}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.2097   & 0.1415  & 32.52\% \\
%         Advection             & 0.3084   & 0.2516  & 18.42\% \\
%         Eikonal               & 0.1203   & 0.0669  & 44.39\% \\
%         Nonlinear Diffusion   & 0.1118   & 0.0618  & 44.72\% \\
%         \bottomrule
%     \end{tabular}

% \end{subtable}


% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=500, train data size=100}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.2020   & 0.1315  & 34.90\% \\
%         Advection             & 0.2997   & 0.2462  & 17.85\% \\
%         Eikonal               & 0.1205   & 0.0671  & 44.32\% \\
%         Nonlinear Diffusion   & 0.1115   & 0.0594  & 46.73\% \\
%         \bottomrule
%     \end{tabular}


% \end{subtable}


% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=600, train data size=100}}
%         \centering
%     \label{tab:Ntr100_Nte100_pts600}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.1911   & 0.1376  & 27.99\% \\
%         Advection             & 0.2868   & 0.2453  & 14.47\% \\
%         Eikonal               & 0.1199   & 0.0665  & 44.54\% \\
%         Nonlinear Diffusion   & 0.1093   & 0.0553  & 49.41\% \\
%         \bottomrule
%     \end{tabular}


% \end{subtable}

% \end{table*}

% \begin{table*}
    

% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=700, train data size=100}}
%         \centering

%     \label{tab:Ntr100_Nte100_pts700}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.1874   & 0.1235  & 34.10\% \\
%         Advection             & 0.2972   & 0.2421  & 18.54\% \\
%         Eikonal               & 0.1159   & 0.0635  & 45.21\% \\
%         Nonlinear Diffusion   & 0.1101   & 0.0507  & 53.95\% \\
%         \bottomrule
%     \end{tabular}
    


% \end{subtable}

% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=800, train data size=100}}
%         \centering

%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}      & GKN    & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow            & 0.1788 & 0.1325 & 25.89\%         \\
%     Advection             & 0.3083 & 0.2408 & 21.89\%         \\
%     Eikonal               & 0.1148 & 0.0625 & 45.56\%         \\
%     Nonlinear Diffusion   & 0.1073 & 0.0527 & 50.89\%         \\
%     \bottomrule
%   \end{tabular}


% \end{subtable}



%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=900, train data size=100}}
%         \centering

%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}      & GKN    & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow            & 0.1777 & 0.1289 & 27.46\%         \\
%     Advection             & 0.2926 & 0.2310 & 21.05\%         \\
%     Eikonal               & 0.1173 & 0.0655 & 44.16\%         \\
%     Nonlinear Diffusion   & 0.1054 & 0.0463 & 56.07\%         \\
%     \bottomrule
%   \end{tabular}


% \end{subtable}



%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=1000, train data size=100}}
%         \centering

%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}      & GKN    & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow            & 0.1748 & 0.1147 & 34.38\%         \\
%     Advection             & 0.2886 & 0.2350 & 18.57\%         \\
%     Eikonal               & 0.1168 & 0.0643 & 44.95\%         \\
%     Nonlinear Diffusion   & 0.1044 & 0.0439 & 57.95\%         \\
%     \bottomrule
%   \end{tabular}
  


% \end{subtable}



% %     \begin{subtable}{\textwidth}
% %         \caption{\small \textit{Sample density=1100, train data size=100}}
% %         \centering

% %   \begin{tabular}{@{}lccc@{}}
% %     \toprule
% %     \textit{Dataset}      & GKN    & Ours   & Error Reduction \\ 
% %     \midrule
% %     Darcy Flow            & 0.1669 & 0.1235 & 26.00\%         \\
% %     Advection             & 0.2919 & 0.2375 & 18.64\%         \\
% %     Eikonal               & 0.1187 & 0.0670 & 43.56\%         \\
% %     Nonlinear Diffusion   & 0.1013 & 0.0490 & 51.63\%         \\
% %     \bottomrule
% %   \end{tabular}
  
% % \end{subtable}

% %     \begin{subtable}{\textwidth}
% %         \caption{\small \textit{Sample density=1200, train data size=100}}
% %         \centering

% %   \begin{tabular}{@{}lccc@{}}
% %     \toprule
% %     \textit{Dataset}      & GKN    & Ours   & Error Reduction \\ 
% %     \midrule
% %     Darcy Flow            & 0.1604 & 0.1223 & 23.75\%         \\
% %     Advection             & 0.2923 & 0.2414 & 17.41\%         \\
% %     Eikonal               & 0.1147 & 0.0666 & 41.94\%         \\
% %     Nonlinear Diffusion   & 0.1012 & 0.0477 & 52.87\%         \\
% %     \bottomrule
% %   \end{tabular}
  
% % \end{subtable}


% %     \begin{subtable}{\textwidth}
% %         \caption{\small \textit{Sample density=1300, train data size=100}}
% %         \centering

% %   \begin{tabular}{@{}lccc@{}}
% %     \toprule
% %     \textit{Dataset}      & GKN    & Ours   & Error Reduction \\ 
% %     \midrule
% %     Darcy Flow            & 0.1585 & 0.1193 & 24.73\%         \\
% %     Advection             & 0.2894 & 0.2312 & 20.11\%         \\
% %     Eikonal               & 0.1152 & 0.0643 & 44.18\%         \\
% %     Nonlinear Diffusion   & 0.1025 & 0.0462 & 54.93\%         \\

% %     \bottomrule
% %   \end{tabular}
  
% % \end{subtable}

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=20, train data size=100}}
%         \centering

%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}      & GKN    & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow            & 0.5027 & 0.4269 & 15.08\%         \\
%     Advection             & 0.9035 & 0.3980 & 55.95\%         \\
%     Eikonal               & 0.1808 & 0.1236 & 31.64\%         \\
%     Nonlinear Diffusion   & 0.2407 & 0.2030 & 15.66\%         \\
%     \bottomrule
%   \end{tabular}
  
% \end{subtable}

% \end{table*}


% \begin{table*}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=30, train data size=100}}
%         \centering

%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.4746   & 0.3776 & 20.44\%         \\
%     Advection                & 0.5409   & 0.4158 & 23.13\%         \\
%     Eikonal                  & 0.1723   & 0.1125 & 34.71\%         \\
%     Nonlinear Diffusion      & 0.2181   & 0.1795 & 17.70\%         \\
%     \bottomrule
%   \end{tabular}
  
% \end{subtable}

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=40, train data size=100}}
%         \centering

%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.4572   & 0.3328 & 27.21\%         \\
%     Advection                & 0.4563   & 0.3773 & 17.31\%         \\
%     Eikonal                  & 0.1671   & 0.1060 & 36.56\%         \\
%     Nonlinear Diffusion      & 0.2133   & 0.1485 & 30.38\%         \\
%     \bottomrule
%   \end{tabular}
  
% \end{subtable}

 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=50, train data size=100}}
%         \centering

%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}        & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow              & 0.4283   & 0.3072 & 28.27\%         \\
%     Advection               & 0.4208   & 0.3747 & 10.96\%          \\
%     Eikonal                 & 0.1620   & 0.0981 & 39.44\%         \\
%     Nonlinear Diffusion     & 0.2066   & 0.1369 & 33.74\%         \\
%     \bottomrule
%   \end{tabular}
  
% \end{subtable}

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=60, train data size=100}}
%         \centering

%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.3995   & 0.2884 & 27.81\%         \\
%     Advection                & 0.3823   & 0.3662 & 4.21\%          \\
%     Eikonal                  & 0.1588   & 0.1020 & 35.77\%         \\
%     Nonlinear Diffusion      & 0.1922   & 0.1248 & 35.07\%         \\
%     \bottomrule
%   \end{tabular}
  
% \end{subtable}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=70, train data size=100}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.3885   & 0.2864 & 26.28\%         \\
%     Advection                & 0.3736   & 0.3626 & 2.94\%          \\
%     Eikonal                  & 0.1546   & 0.0953 & 38.36\%         \\
%     Nonlinear Diffusion      & 0.1876   & 0.1206 & 35.71\%         \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=80, train data size=100}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.3760   & 0.2750 & 26.86\%         \\
%     Advection                & 0.3468   & 0.3368 & 2.88\%          \\
%     Eikonal                  & 0.1472   & 0.0956 & 35.05\%         \\
%     Nonlinear Diffusion      & 0.1851   & 0.1166 & 37.01\%         \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}



%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=90, train data size=100}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.3646   & 0.2572 & 29.46\%         \\
%     Advection                & 0.3422   & 0.3315 & 3.13\%          \\
%     Eikonal                  & 0.1472   & 0.0940 & 36.14\%         \\
%     Nonlinear Diffusion      & 0.1760   & 0.1117 & 36.53\%         \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}




% % \end{table*}


% % \begin{table*}

%         \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=100, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.4122   & 0.2994 & 27.37\%         \\
%     Advection                & 0.4938   & 0.4547 & 7.92\%          \\
%     Eikonal                  & 0.1668   & 0.1102 & 33.93\%         \\
%     Nonlinear Diffusion      & 0.1947   & 0.1161 & 40.37\%         \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}

% \end{table*}

% \begin{table*}

   

%         \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=200, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.3281   & 0.2388 & 27.22\%         \\
%     Advection                & 0.4840   & 0.4420 & 8.68\%          \\
%     Eikonal                  & 0.1429   & 0.1050 & 26.52\%         \\
%     Nonlinear Diffusion      & 0.1714   & 0.0951 & 44.52\%         \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}


%         \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=300, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.2746   & 0.2126 & 22.58\%         \\
%     Advection                & 0.4660   & 0.4178 & 10.34\%         \\
%     Eikonal                  & 0.1390   & 0.0982 & 29.35\%         \\
%     Nonlinear Diffusion      & 0.1589   & 0.0849 & 46.57\%         \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}





%             \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=400, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.2446   & 0.1968 & 19.54\%         \\
%     Advection                & 0.4590   & 0.4005 & 12.75\%         \\
%     Eikonal                  & 0.1396   & 0.0952 & 31.81\%         \\
%     Nonlinear Diffusion      & 0.1536   & 0.0776 & 49.48\%         \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}


%             \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=500, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.2505   & 0.1878 & 25.03\%         \\
%     Advection                & 0.4746   & 0.3609 & 23.96\%         \\
%     Eikonal                  & 0.1355   & 0.0957 & 29.37\%         \\
%     Nonlinear Diffusion      & 0.1389   & 0.0760 & 45.28\%         \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}



%             \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=600, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.2416   & 0.1648 & 31.79\%         \\
%     Advection                & 0.4352   & 0.3661 & 15.88\%         \\
%     Eikonal                  & 0.1323   & 0.0772 & 41.65\%         \\
%     Nonlinear Diffusion      & 0.1441   & 0.0739 & 48.72\%         \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}


%             \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=700, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.2257   & 0.1592 & 29.46\%         \\
%     Advection                & 0.4546   & 0.3747 & 17.58\%         \\
%     Eikonal                  & 0.1294   & 0.0819 & 36.71\%         \\
%     Nonlinear Diffusion      & 0.1424   & 0.0731 & 48.67\%         \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}


%             \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=800, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.2120   & 0.1572 & 25.85\%         \\
%     Advection                & 0.4558   & 0.3789 & 16.87\%         \\
%     Eikonal                  & 0.1304   & 0.0761 & 41.64\%         \\
%     Nonlinear Diffusion      & 0.1413   & 0.0701 & 50.39\%         \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}



%             \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=900, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.2068   & 0.1503 & 27.32\%         \\
%     Advection                & 0.4292   & 0.3560 & 17.05\%         \\
%     Eikonal                  & 0.1306   & 0.0805 & 38.36\%         \\
%     Nonlinear Diffusion      & 0.1441   & 0.0691 & 52.05\%         \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}

% \end{table*}



% \begin{table*}


%             \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=1000, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.2257   & 0.1592 & 29.46\%         \\
%     Advection                & 0.4546   & 0.3747 & 17.58\%         \\
%     Eikonal                  & 0.1294   & 0.0819 & 36.71\%         \\
%     Nonlinear Diffusion      & 0.1424   & 0.0731 & 48.67\%         \\
%     \bottomrule
%   \end{tabular}

% \end{subtable}



%             \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=20, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.5527   & 0.4567 & 17.37\%         \\
%     Advection                & 0.9735   & 0.5219 & 46.39\%         \\
%     Eikonal                  & 0.1868   & 0.1451 & 22.32\%         \\
%     Nonlinear Diffusion      & 0.2892   & 0.2297 & 20.57\%         \\
%     \bottomrule
%   \end{tabular}


% \end{subtable}



%               \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=30, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.5180   & 0.4114 & 20.58\%         \\
%     Advection                & 0.7502   & 0.4694 & 37.43\%         \\
%     Eikonal                  & 0.1847   & 0.1354 & 26.69\%         \\
%     Nonlinear Diffusion      & 0.2638   & 0.1867 & 29.23\%         \\
%     \bottomrule
%   \end{tabular}


% \end{subtable}


%               \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=40, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.5074   & 0.3840 & 24.32\%         \\
%     Advection                & 0.6341   & 0.4714 & 25.66\%         \\
%     Eikonal                  & 0.1833   & 0.1234 & 32.68\%         \\
%     Nonlinear Diffusion      & 0.2464   & 0.1563 & 36.57\%         \\
%     \bottomrule
%   \end{tabular}


% \end{subtable}



%               \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=50, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.4819   & 0.3546 & 26.42\%         \\
%     Advection                & 0.5321   & 0.4897 & 7.97\%          \\
%     Eikonal                  & 0.1798   & 0.1194 & 33.59\%         \\
%     Nonlinear Diffusion      & 0.2417   & 0.1439 & 40.46\%         \\
%     \bottomrule
%   \end{tabular}


% \end{subtable}


%               \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=60, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.4664   & 0.3308 & 29.07\%         \\
%     Advection                & 0.5688   & 0.4993 & 12.22\%         \\
%     Eikonal                  & 0.1777   & 0.1181 & 33.54\%         \\
%     Nonlinear Diffusion      & 0.2349   & 0.1318 & 43.89\%         \\
%     \bottomrule
%   \end{tabular}


% \end{subtable}


%               \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=70, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN      & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.4518   & 0.3176 & 29.70\%         \\
%     Advection                & 0.5410   & 0.4766 & 11.90\%         \\
%     Eikonal                  & 0.1663   & 0.1147 & 31.03\%         \\
%     Nonlinear Diffusion      & 0.2195   & 0.1294 & 41.05\%         \\
%     \bottomrule
%   \end{tabular}


% \end{subtable}

%               \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=80, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN      & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.4558   & 0.2994 & 34.31\%         \\
%     Advection                & 0.5175   & 0.4535 & 12.37\%         \\
%     Eikonal                  & 0.1642   & 0.1132 & 31.06\%         \\
%     Nonlinear Diffusion      & 0.2127   & 0.1225 & 42.41\%         \\
%     \bottomrule
%   \end{tabular}


% \end{subtable}

% \end{table*}


% \begin{table*}



%               \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=90, train data size=40}}
%         \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \textit{Dataset}         & GKN      & Ours   & Error Reduction \\ 
%     \midrule
%     Darcy Flow               & 0.4378   & 0.2791 & 36.25\%         \\
%     Advection                & 0.5039   & 0.4452 & 11.65\%         \\
%     Eikonal                  & 0.1706   & 0.1122 & 34.23\%         \\
%     Nonlinear Diffusion      & 0.1996   & 0.1179 & 40.93\%         \\
%     \bottomrule
%   \end{tabular}


% \end{subtable}



% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=100, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset} & GKN & Ours & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.4404 & 0.3705 & 15.87\% \\
%         Advection             & 0.5708 & 0.4977 & 12.81\% \\
%         Eikonal               & 0.1825 & 0.1047 & 42.63\% \\
%         Nonlinear Diffusion   & 0.2168 & 0.1234 & 43.08\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable}


% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=200, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}             & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow          & 0.3651   & 0.2275  & 37.69\% \\
%         Advection           & 0.5242   & 0.4123  & 21.35\% \\
%         Eikonal             & 0.1633   & 0.0981  & 39.93\% \\
%         Nonlinear Diffusion & 0.1919   & 0.1024  & 46.64\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}


% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=300, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}             & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow          & 0.3168   & 0.1906  & 39.83\% \\
%         Advection           & 0.5841   & 0.4191  & 28.25\% \\
%         Eikonal             & 0.1701   & 0.0921  & 45.86\% \\
%         Nonlinear Diffusion & 0.1709   & 0.0873  & 48.92\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}


% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=400, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}             & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow          & 0.2938   & 0.1864  & 36.56\% \\
%         Advection           & 0.5157   & 0.4090  & 20.69\% \\
%         Eikonal             & 0.1684   & 0.0908  & 46.08\% \\
%         Nonlinear Diffusion & 0.1683   & 0.0815  & 51.57\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}



% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=500, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}             & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow          & 0.2810   & 0.1772  & 36.94\% \\
%         Advection           & 0.5915   & 0.4089  & 30.87\% \\
%         Eikonal             & 0.1582   & 0.0901  & 43.05\% \\
%         Nonlinear Diffusion & 0.1588   & 0.0773  & 51.32\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}



% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=600, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}             & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow          & 0.2702   & 0.1646  & 39.08\% \\
%         Advection           & 0.5344   & 0.4109  & 23.11\% \\
%         Eikonal             & 0.1553   & 0.0776  & 50.03\% \\
%         Nonlinear Diffusion & 0.1582   & 0.0709  & 55.18\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}



% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=700, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.2618   & 0.1659  & 36.63\% \\
%         Advection             & 0.5387   & 0.4172  & 22.55\% \\
%         Eikonal               & 0.1550   & 0.0801  & 48.32\% \\
%         Nonlinear Diffusion   & 0.1547   & 0.0734  & 52.55\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}



% \end{table*}

% \begin{table*}




% \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=800, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.2524   & 0.1576  & 37.56\% \\
%         Advection             & 0.5527   & 0.4148  & 24.95\% \\
%         Eikonal               & 0.1541   & 0.0756  & 50.94\% \\
%         Nonlinear Diffusion   & 0.1495   & 0.0706  & 52.78\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}



%   \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=900, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.2454   & 0.1587  & 35.33\% \\
%         Advection             & 0.4994   & 0.4074  & 18.42\% \\
%         Eikonal               & 0.1550   & 0.0760  & 50.97\% \\
%         Nonlinear Diffusion   & 0.1519   & 0.0683  & 55.04\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}


%   \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=1000, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.2375   & 0.1554  & 34.57\% \\
%         Advection             & 0.5353   & 0.3707  & 30.75\% \\
%         Eikonal               & 0.1530   & 0.0803  & 47.52\% \\
%         Nonlinear Diffusion   & 0.1520   & 0.0747  & 50.86\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}


%   \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=20, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.5574   & 0.4984  & 10.58\% \\
%         Advection             & 0.9881   & 0.4798  & 51.44\% \\
%         Eikonal               & 0.1929   & 0.1402  & 27.32\% \\
%         Nonlinear Diffusion   & 0.2958   & 0.2365  & 20.05\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}


%   \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=30, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.5203   & 0.4509  & 13.34\% \\
%         Advection             & 0.7924   & 0.4655  & 41.25\% \\
%         Eikonal               & 0.1920   & 0.1313  & 31.61\% \\
%         Nonlinear Diffusion   & 0.2761   & 0.1878  & 31.98\% \\
%         \bottomrule
%     \end{tabular}


    
% \end{subtable}

%   \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=40, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.5028   & 0.4190  & 16.67\% \\
%         Advection             & 0.7468   & 0.4642  & 37.84\% \\
%         Eikonal               & 0.1893   & 0.1200  & 36.61\% \\
%         Nonlinear Diffusion   & 0.2581   & 0.1647  & 36.19\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}


%   \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=50, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.4881   & 0.3902  & 20.06\% \\
%         Advection             & 0.6657   & 0.4580  & 31.20\% \\
%         Eikonal               & 0.1852   & 0.1174  & 36.61\% \\
%         Nonlinear Diffusion   & 0.2512   & 0.1523  & 39.37\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}


%   \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=60, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.4667   & 0.3733  & 20.01\% \\
%         Advection             & 0.6622   & 0.4537  & 31.49\% \\
%         Eikonal               & 0.1801   & 0.1162  & 35.48\% \\
%         Nonlinear Diffusion   & 0.2423   & 0.1408  & 41.89\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}

% \end{table*}


% \begin{table*}



%   \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=70, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.4576   & 0.3565  & 22.09\% \\
%         Advection             & 0.5756   & 0.4583  & 20.38\% \\
%         Eikonal               & 0.1757   & 0.1138  & 35.23\% \\
%         Nonlinear Diffusion   & 0.2353   & 0.1369  & 41.82\% \\
%         \bottomrule
%     \end{tabular}

    
% \end{subtable}



%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=80, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.4568   & 0.3394  & 25.70\% \\
%         Advection             & 0.5646   & 0.4460  & 21.01\% \\
%         Eikonal               & 0.1803   & 0.1115  & 38.16\% \\
%         Nonlinear Diffusion   & 0.2219   & 0.1295  & 41.64\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable}  

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=90, train data size=30}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.4513   & 0.3225  & 28.54\% \\
%         Advection             & 0.5889   & 0.4470  & 24.10\% \\
%         Eikonal               & 0.1817   & 0.1088  & 40.12\% \\
%         Nonlinear Diffusion   & 0.2135   & 0.1279  & 40.09\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable}  

% \end{table*}


% \begin{table*}

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=100, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts100}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}        & GKN     & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow              & 0.4790  & 0.3986  & 16.78\% \\
%         Advection               & 0.8125  & 0.5498  & 32.33\% \\
%         Eikonal                 & 0.1848  & 0.1115  & 39.66\% \\
%         Nonlinear Diffusion     & 0.2284  & 0.1332  & 41.68\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable}  

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=200, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts200}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.3937   & 0.2812  & 28.58\% \\
%         Advection             & 0.8552   & 0.5004  & 41.49\% \\
%         Eikonal               & 0.1780   & 0.1069  & 39.94\% \\
%         Nonlinear Diffusion   & 0.2056   & 0.1060  & 48.44\% \\
%         \bottomrule
%     \end{tabular}

% \end{subtable}  

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=300, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts300}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.3414   & 0.2416  & 29.23\% \\
%         Advection             & 0.7282   & 0.5323  & 26.90\% \\
%         Eikonal               & 0.1757   & 0.1066  & 39.33\% \\
%         Nonlinear Diffusion   & 0.1923   & 0.0920  & 52.16\% \\
%         \bottomrule
%     \end{tabular}

% \end{subtable}  



    
%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=400, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts400}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.3291   & 0.2471  & 24.92\% \\
%         Advection             & 0.7667   & 0.5317  & 30.65\% \\
%         Eikonal               & 0.1716   & 0.1058  & 38.34\% \\
%         Nonlinear Diffusion   & 0.1831   & 0.0847  & 53.74\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=500, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts500}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.3285   & 0.2247  & 31.60\% \\
%         Advection             & 1.0101   & 0.5431  & 46.23\% \\
%         Eikonal               & 0.1703   & 0.1060  & 37.76\% \\
%         Nonlinear Diffusion   & 0.1783   & 0.0801  & 55.08\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=600, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts600}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}        & GKN     & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow              & 0.3030  & 0.2362  & 22.05\% \\
%         Advection               & 0.7948  & 0.5754  & 27.60\% \\
%         Eikonal                 & 0.1739  & 0.1073  & 38.30\% \\
%         Nonlinear Diffusion     & 0.1780  & 0.0781  & 56.12\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=700, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts700}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}        & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow              & 0.3001   & 0.2332  & 22.29\% \\
%         Advection               & 0.7928   & 0.5594  & 29.44\% \\
%         Eikonal                 & 0.1682   & 0.1038  & 38.29\% \\
%         Nonlinear Diffusion     & 0.1755   & 0.0731  & 58.35\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 



% \end{table*}



% \begin{table*}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=800, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts800}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}        & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow              & 0.2841   & 0.2303  & 18.94\% \\
%         Advection               & 0.8037   & 0.4799  & 40.29\% \\
%         Eikonal                 & 0.1696   & 0.1038  & 38.80\% \\
%         Nonlinear Diffusion     & 0.1749   & 0.0728  & 58.38\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 






%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=900, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts900}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}        & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow              & 0.2787   & 0.2215  & 20.52\% \\
%         Advection               & 0.7267   & 0.4866  & 33.04\% \\
%         Eikonal                 & 0.1705   & 0.1059  & 37.89\% \\
%         Nonlinear Diffusion     & 0.1755   & 0.0740  & 57.83\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=1000, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts1000}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours     & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.2660   & 0.2297   & 13.65\% \\
%         Advection             & 0.7421   & 0.5268   & 29.01\% \\
%         Eikonal               & 0.1697   & 0.1059   & 37.60\% \\
%         Nonlinear Diffusion   & 0.1716   & 0.0757   & 55.89\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=20, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts20}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}        & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow              & 0.5909   & 0.5363  & 9.24\%  \\
%         Advection               & 1.0704   & 0.5114  & 52.22\% \\
%         Eikonal                 & 0.1985   & 0.1543  & 22.27\% \\
%         Nonlinear Diffusion     & 0.3053   & 0.2403  & 21.29\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 



%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=30, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts30}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}        & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow              & 0.5712   & 0.5131  & 10.17\% \\
%         Advection               & 1.0391   & 0.4973  & 52.14\% \\
%         Eikonal                 & 0.1941   & 0.1377  & 29.06\% \\
%         Nonlinear Diffusion     & 0.2804   & 0.2003  & 28.57\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=40, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts40}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.5493   & 0.4674  & 14.91\% \\
%         Advection             & 0.9612   & 0.5189  & 46.02\% \\
%         Eikonal               & 0.1916   & 0.1255  & 34.50\% \\
%         Nonlinear Diffusion   & 0.2655   & 0.1755  & 33.90\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=50, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts50}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}        & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow              & 0.5221   & 0.4445  & 14.86\% \\
%         Advection               & 0.9652   & 0.5618  & 41.79\% \\
%         Eikonal                 & 0.1880   & 0.1191  & 36.65\% \\
%         Nonlinear Diffusion     & 0.2525   & 0.1661  & 34.22\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=60, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts60}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}        & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow              & 0.5013   & 0.4251  & 15.20\% \\
%         Advection               & 0.8556   & 0.5541  & 35.24\% \\
%         Eikonal                 & 0.1864   & 0.1192  & 36.05\% \\
%         Nonlinear Diffusion     & 0.2459   & 0.1580  & 35.75\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


% \end{table*}



% \begin{table*}



%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=70, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts70}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.4975   & 0.3965  & 20.30\% \\
%         Advection             & 0.8128   & 0.5524  & 32.04\% \\
%         Eikonal               & 0.1838   & 0.1154  & 37.21\% \\
%         Nonlinear Diffusion   & 0.2420   & 0.1498  & 38.10\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=80, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts80}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}        & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow              & 0.4937   & 0.3709  & 24.87\% \\
%         Advection               & 0.7770   & 0.5318  & 31.56\% \\
%         Eikonal                 & 0.1835   & 0.1170  & 36.24\% \\
%         Nonlinear Diffusion     & 0.2387   & 0.1401  & 41.31\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=90, train data size=20}}
%         \centering
%     \label{tab:Ntr20_Nte100_pts90}
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.4920   & 0.3638  & 26.06\% \\
%         Advection             & 0.8157   & 0.5334  & 34.61\% \\
%         Eikonal               & 0.1847   & 0.1140  & 38.28\% \\
%         Nonlinear Diffusion   & 0.2313   & 0.1329  & 42.54\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 



% % \end{table*}



% % \begin{table*}
    
% % \end{table*}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=100, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.5692   & 0.4673  & 17.90\% \\
%         Advection             & 1.0858   & 0.6738  & 37.94\% \\
%         Eikonal               & 0.2061   & 0.1402  & 31.98\% \\
%         Nonlinear Diffusion   & 0.2531   & 0.1691  & 33.19\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=200, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.4593   & 0.3431  & 25.30\% \\
%         Advection             & 1.0516   & 0.6407  & 39.07\% \\
%         Eikonal               & 0.2018   & 0.1276  & 36.77\% \\
%         Nonlinear Diffusion   & 0.2500   & 0.1605  & 35.80\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=300, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.4014   & 0.3233  & 19.46\% \\
%         Advection             & 0.9618   & 0.6674  & 30.61\% \\
%         Eikonal               & 0.1955   & 0.1246  & 36.27\% \\
%         Nonlinear Diffusion   & 0.2548   & 0.1498  & 41.21\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=400, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.3750   & 0.3109  & 17.09\% \\
%         Advection             & 1.0257   & 0.6733  & 34.36\% \\
%         Eikonal               & 0.1913   & 0.1203  & 37.11\% \\
%         Nonlinear Diffusion   & 0.2430   & 0.1411  & 41.93\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=500, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.3764   & 0.2842  & 24.50\% \\
%         Advection             & 0.9785   & 0.7011  & 28.35\% \\
%         Eikonal               & 0.1905   & 0.1155  & 39.37\% \\
%         Nonlinear Diffusion   & 0.2383   & 0.1464  & 38.56\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


% \end{table*}


% \begin{table*}
    

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=600, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.3645   & 0.2886  & 20.82\% \\
%         Advection             & 1.0162   & 0.7271  & 28.45\% \\
%         Eikonal               & 0.1929   & 0.1255  & 34.94\% \\
%         Nonlinear Diffusion   & 0.2360   & 0.1440  & 38.98\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=700, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.3522   & 0.2768  & 21.41\% \\
%         Advection             & 0.9918   & 0.6590  & 33.56\% \\
%         Eikonal               & 0.1929   & 0.1180  & 38.83\% \\
%         Nonlinear Diffusion   & 0.2289   & 0.1363  & 40.45\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=800, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.3400   & 0.2781  & 18.21\% \\
%         Advection             & 1.0006   & 0.7109  & 28.95\% \\
%         Eikonal               & 0.1909   & 0.1210  & 36.62\% \\
%         Nonlinear Diffusion   & 0.2304   & 0.1406  & 38.98\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=900, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}        & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow              & 0.3356   & 0.2812  & 16.21\% \\
%         Advection               & 1.0374   & 0.6862  & 33.85\% \\
%         Eikonal                 & 0.1913   & 0.1245  & 34.92\% \\
%         Nonlinear Diffusion     & 0.2319   & 0.1420  & 38.77\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=1000, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.3345   & 0.2787  & 16.68\% \\
%         Advection             & 1.0026   & 0.6668  & 33.49\% \\
%         Eikonal               & 0.1956   & 0.1286  & 34.25\% \\
%         Nonlinear Diffusion   & 0.2346   & 0.1204  & 48.68\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=20, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.6578   & 0.5963  & 9.35\% \\
%         Advection             & 1.1149   & 0.7329  & 34.26\% \\
%         Eikonal               & 0.2144   & 0.1797  & 16.18\% \\
%         Nonlinear Diffusion   & 0.3280   & 0.3074  & 6.28\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=30, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.6580   & 0.5529  & 15.97\% \\
%         Advection             & 1.1036   & 0.6746  & 38.87\% \\
%         Eikonal               & 0.2073   & 0.1606  & 22.53\% \\
%         Nonlinear Diffusion   & 0.3017   & 0.2735  & 9.35\%  \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=40, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.6207   & 0.5169  & 16.72\% \\
%         Advection             & 1.1147   & 0.6941  & 37.73\% \\
%         Eikonal               & 0.2090   & 0.1521  & 27.22\% \\
%         Nonlinear Diffusion   & 0.2920   & 0.2439  & 16.47\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 

% \end{table*}


% \begin{table*}



%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=50, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.5909   & 0.4944  & 16.33\% \\
%         Advection             & 1.0714   & 0.6219  & 41.95\% \\
%         Eikonal               & 0.2063   & 0.1498  & 27.39\% \\
%         Nonlinear Diffusion   & 0.2788   & 0.2048  & 26.54\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=60, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.5624   & 0.4762  & 15.33\% \\
%         Advection             & 1.1333   & 0.6342  & 44.04\% \\
%         Eikonal               & 0.2051   & 0.1483  & 27.69\% \\
%         Nonlinear Diffusion   & 0.2751   & 0.1963  & 28.64\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=70, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.5629   & 0.4682  & 16.82\% \\
%         Advection             & 1.1024   & 0.6654  & 39.64\% \\
%         Eikonal               & 0.2039   & 0.1450  & 28.89\% \\
%         Nonlinear Diffusion   & 0.2609   & 0.1776  & 31.93\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=80, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.5795   & 0.4561  & 21.29\% \\
%         Advection             & 1.0573   & 0.6365  & 39.80\% \\
%         Eikonal               & 0.2041   & 0.1412  & 30.82\% \\
%         Nonlinear Diffusion   & 0.2600   & 0.1777  & 31.65\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Sample density=90, train data size=10}}
%         \centering
%     \begin{tabular}{lccc}
%         \toprule
%         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
%         \midrule
%         Darcy Flow            & 0.5824   & 0.4362  & 25.10\% \\
%         Advection             & 1.1247   & 0.6612  & 41.21\% \\
%         Eikonal               & 0.2047   & 0.1401  & 31.56\% \\
%         Nonlinear Diffusion   & 0.2597   & 0.1693  & 34.81\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{subtable} 




% \end{table*}



% % \begin{table*}

% %         \begin{subtable}{\textwidth}
% %         \caption{\small \textit{Sample density=50, train data size=10}}
% %         \centering
% %     \begin{tabular}{lccc}
% %         \toprule
% %         \textit{Dataset}      & GKN      & Ours    & Error Reduction \\
% %         \midrule
% %         Darcy Flow            & 0.5909   & 0.4944  & 16.33\% \\
% %         Advection             & 1.0714   & 0.6219  & 41.95\% \\
% %         Eikonal               & 0.2063   & 0.1498  & 27.39\% \\
% %         Nonlinear Diffusion   & 0.2788   & 0.2048  & 26.54\% \\
% %         \bottomrule
% %     \end{tabular}

    
% % \end{table*}


% \begin{table*}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Darcy Flow test errors trained on 100 training data size across various sampling density.}}
%         \centering

% \label{tab:darcy_flow_ntr100_density}
% \begin{tabular}{cccc}
% \toprule
% Density & GKN    & Ours   & Error Reduction\\
% \midrule
% 20    & 0.5027 & 0.4073 & 18.98\% \\
% 30    & 0.4746 & 0.3663 & 22.82\% \\
% 40    & 0.4572 & 0.3328 & 27.21\% \\
% 50    & 0.4283 & 0.3072 & 28.27\% \\
% 60    & 0.3995 & 0.2711 & 32.14\% \\
% 70    & 0.3885 & 0.2710 & 30.24\% \\
% 80    & 0.3760 & 0.2566 & 31.76\% \\
% 90    & 0.3646 & 0.2420 & 33.63\% \\
% 100   & 0.3402 & 0.2349 & 30.95\% \\
% 200   & 0.2633 & 0.1878 & 28.67\% \\
% 300   & 0.2355 & 0.1479 & 37.20\% \\
% 400   & 0.2097 & 0.1415 & 32.52\% \\
% 500   & 0.2020 & 0.1315 & 34.90\% \\
% 600   & 0.1911 & 0.1242 & 35.01\% \\
% 700   & 0.1874 & 0.1235 & 34.10\% \\
% 800   & 0.1788 & 0.1226 & 31.43\% \\
% 900   & 0.1777 & 0.1168 & 34.27\% \\
% 1000  & 0.1748 & 0.1147 & 34.38\% \\
% \bottomrule
% \end{tabular}
    

    
%     \end{subtable}

% \end{table*}


% \begin{table*}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Eikonal test errors trained on 100 training data size across various sampling density.}}
%         \centering

%     \begin{tabular}{cccc}
%         \toprule
%         \textbf{Density} & \textbf{GKN} & \textbf{Ours} & \textbf{Error Reduction} \\
%         \midrule
% 20   & 0.1808 & 0.1236 & 31.64\% \\
% 30   & 0.1723 & 0.1125 & 34.71\% \\
% 40   & 0.1671 & 0.1060 & 36.56\% \\
% 50   & 0.1620 & 0.1012 & 37.53\% \\
% 60   & 0.1588 & 0.1020 & 35.77\% \\
% 70   & 0.1546 & 0.0953 & 38.36\% \\
% 80   & 0.1472 & 0.0956 & 35.05\% \\
% 90   & 0.1472 & 0.0940 & 36.14\% \\
% 100  & 0.1442 & 0.0857 & 40.57\% \\
% 200  & 0.1325 & 0.0745 & 43.77\% \\
% 300  & 0.1238 & 0.0664 & 46.37\% \\
% 400  & 0.1203 & 0.0669 & 44.39\% \\
% 500  & 0.1205 & 0.0671 & 44.32\% \\
% 600  & 0.1199 & 0.0665 & 44.54\% \\
% 700  & 0.1159 & 0.0676 & 41.67\% \\
% 800  & 0.1148 & 0.0625 & 45.56\% \\
% 900  & 0.1173 & 0.0655 & 44.16\% \\
% 1000 & 0.1168 & 0.0643 & 44.95\% \\
%         \bottomrule
%     \end{tabular}

    
    
%     \end{subtable}



%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Nonlinear Diffusion test errors trained on 100 training data size across various sampling density.}}
%         \centering

% \label{tab:nonlinear_diffusion_ntr100_sampling_density}
% \begin{tabular}{cccc}
% \toprule
% Density & GKN    & Ours   & Error Reduction (\%) \\
% \midrule
% 20    & 0.2407 & 0.1958 & 18.65\% \\
% 30    & 0.2181 & 0.1795 & 17.70\% \\
% 40    & 0.2133 & 0.1446 & 32.21\% \\
% 50    & 0.2066 & 0.1369 & 33.74\% \\
% 60    & 0.1922 & 0.1248 & 35.07\% \\
% 70    & 0.1876 & 0.1206 & 35.71\% \\
% 80    & 0.1851 & 0.1067 & 42.36\% \\
% 90    & 0.1760 & 0.0995 & 43.47\% \\
% 100   & 0.1689 & 0.0947 & 43.93\% \\
% 200   & 0.1415 & 0.0755 & 46.64\% \\
% 300   & 0.1245 & 0.0674 & 45.86\% \\
% 400   & 0.1118 & 0.0618 & 44.72\% \\
% 500   & 0.1115 & 0.0594 & 46.73\% \\
% 600   & 0.1093 & 0.0553 & 49.41\% \\
% 700   & 0.1101 & 0.0507 & 53.95\% \\
% 800   & 0.1073 & 0.0469 & 56.29\% \\
% 900   & 0.1054 & 0.0463 & 56.07\% \\
% 1000  & 0.1044 & 0.0439 & 57.95\% \\
% \bottomrule
% \end{tabular}
    
    
%     \end{subtable}



%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Advection test errors trained on 100 training data size across various sampling density.}}
%         \centering

%     \begin{tabular}{cccc}
%         \toprule
%         \textbf{Density} & \textbf{GKN} & \textbf{Ours} & \textbf{Error Reduction} \\
%         \midrule
% 20    & 0.9035 & 0.3980 & 55.95\% \\
% 30    & 0.5409 & 0.4158 & 23.13\% \\
% 40    & 0.4563 & 0.3773 & 17.31\% \\
% 50    & 0.4208 & 0.3747 &  10.96\% \\
% 60    & 0.3823 & 0.3662 &  4.21\% \\
% 70    & 0.3736 & 0.3626 &  2.94\% \\
% 80    & 0.3468 & 0.3368 &  2.88\% \\
% 90    & 0.3422 & 0.3315 &  3.13\% \\
% 100   & 0.3446 & 0.3216 &  6.67\% \\
% 200   & 0.3150 & 0.2880 &  8.57\% \\
% 300   & 0.3017 & 0.2537 & 15.91\% \\
% 400   & 0.3084 & 0.2516 & 18.42\% \\
% 500   & 0.2997 & 0.2462 & 17.85\% \\
% 600   & 0.2868 & 0.2453 & 14.47\% \\
% 700   & 0.2972 & 0.2421 & 18.54\% \\
% 800   & 0.3083 & 0.2408 & 21.89\% \\
% 900   & 0.2926 & 0.2310 & 21.05\% \\
% 1000  & 0.2886 & 0.2350 & 18.57\% \\
%         \bottomrule
%     \end{tabular}
    
    
%     \end{subtable}

%     \end{table*}



% \begin{table*}

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Darcy Flow test errors trained on 50 training data size across various sampling density.}}
%         \centering

%      \begin{tabular}{cccc}
%         \toprule
%         \textbf{Density} & \textbf{GKN} & \textbf{Ours} & \textbf{Error Reduction} \\
%         \midrule
% 20    & 0.5690 & 0.4615 & 18.89\% \\
% 30    & 0.5192 & 0.4156 & 19.95\% \\
% 40    & 0.5085 & 0.4112 & 19.13\% \\
% 50    & 0.4783 & 0.3790 & 20.76\% \\
% 60    & 0.4467 & 0.2884 & 35.44\% \\
% 70    & 0.4328 & 0.3370 & 22.13\% \\
% 80    & 0.4310 & 0.3137 & 27.22\% \\
% 90    & 0.4099 & 0.3024 & 26.23\% \\
% 100   & 0.4068 & 0.2918 & 28.27\% \\
% 200   & 0.3092 & 0.2182 & 29.43\% \\
% 300   & 0.2673 & 0.1958 & 26.75\% \\
% 400   & 0.2421 & 0.1860 & 23.17\% \\
% 500   & 0.2326 & 0.1761 & 24.29\% \\
% 600   & 0.2173 & 0.1671 & 23.10\% \\
% 700   & 0.2114 & 0.1644 & 22.23\% \\
% 800   & 0.1990 & 0.1623 & 18.44\% \\
% 900   & 0.1901 & 0.1611 & 15.26\% \\
% 1000  & 0.1890 & 0.1597 & 15.50\% \\
%         \bottomrule
%     \end{tabular}

    
%     \end{subtable}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Eikonal test errors trained on 50 training data size across various sampling density.}}
%         \centering


%     \begin{tabular}{cccc}
%         \toprule
%         \textbf{Density} & \textbf{GKN} & \textbf{Ours} & \textbf{Error Reduction} \\
%         \midrule
% 20    & 0.1908 & 0.1505 & 21.12\% \\
% 30    & 0.1870 & 0.1323 & 29.25\% \\
% 40    & 0.1839 & 0.1256 & 31.70\% \\
% 50    & 0.1764 & 0.1234 & 30.05\% \\
% 60    & 0.1739 & 0.1195 & 31.28\% \\
% 70    & 0.1670 & 0.1188 & 28.86\% \\
% 80    & 0.1640 & 0.1117 & 31.89\% \\
% 90    & 0.1643 & 0.1083 & 34.08\% \\
% 100   & 0.1592 & 0.0988 & 37.94\% \\
% 200   & 0.1386 & 0.0873 & 37.01\% \\
% 300   & 0.1380 & 0.0958 & 30.58\% \\
% 400   & 0.1341 & 0.0928 & 30.80\% \\
% 500   & 0.1292 & 0.0928 & 28.17\% \\
% 600   & 0.1309 & 0.0932 & 28.80\% \\
% 700   & 0.1299 & 0.0713 & 45.11\% \\
% 800   & 0.1288 & 0.0902 & 29.97\% \\
% 900   & 0.1300 & 0.0893 & 31.31\% \\
% 1000  & 0.1273 & 0.0895 & 29.69\% \\
%         \bottomrule
%     \end{tabular}

    
    
%     \end{subtable}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Nonlinear Diffusion test errors trained on 50 training data size across various sampling density.}}
%         \centering

%     \begin{tabular}{cccc}
%         \toprule
%         \textbf{Density} & \textbf{GKN} & \textbf{Ours} & \textbf{Error Reduction} \\
%         \midrule
% 20    & 0.2817 & 0.2202 & 21.83\% \\
% 30    & 0.2554 & 0.1858 & 27.25\% \\
% 40    & 0.2413 & 0.1485 & 38.46\% \\
% 50    & 0.2339 & 0.1472 & 37.07\% \\
% 60    & 0.2266 & 0.1387 & 38.79\% \\
% 70    & 0.2117 & 0.1339 & 36.75\% \\
% 80    & 0.2081 & 0.1250 & 39.93\% \\
% 90    & 0.1955 & 0.1189 & 39.18\% \\
% 100   & 0.1903 & 0.1157 & 39.20\% \\
% 200   & 0.1597 & 0.0932 & 41.64\% \\
% 300   & 0.1506 & 0.0818 & 45.68\% \\
% 400   & 0.1390 & 0.0766 & 44.89\% \\
% 500   & 0.1301 & 0.0733 & 43.66\% \\
% 600   & 0.1349 & 0.0716 & 46.92\% \\
% 700   & 0.1308 & 0.0677 & 48.24\% \\
% 800   & 0.1284 & 0.0652 & 49.22\% \\
% 900   & 0.1258 & 0.0621 & 50.64\% \\
% 1000  & 0.1218 & 0.0532 & 56.32\% \\
%         \bottomrule
%     \end{tabular}
    
%     \end{subtable}


% \end{table*}

% \begin{table*}
    



%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Advection test errors trained on 50 training data size across various sampling density.}}
%         \centering


%        \begin{tabular}{cccc}
%         \toprule
%         \textbf{Density} & \textbf{GKN} & \textbf{Ours} & \textbf{Error Reduction} \\
%         \midrule
% 20    & 0.8899 & 0.5043 & 43.33\% \\
% 30    & 0.6991 & 0.4772 & 31.74\% \\
% 40    & 0.5983 & 0.4845 & 19.02\% \\
% 50    & 0.5569 & 0.4639 & 16.70\% \\
% 60    & 0.6016 & 0.4653 & 22.66\% \\
% 70    & 0.4733 & 0.4400 &  7.04\% \\
% 80    & 0.4585 & 0.4516 &  1.50\% \\
% 90    & 0.4559 & 0.4238 &  7.04\% \\
% 100   & 0.4467 & 0.4130 &  7.54\% \\
% 200   & 0.4156 & 0.4055 &  2.43\% \\
% 300   & 0.4132 & 0.3882 &  6.05\% \\
% 400   & 0.4126 & 0.3658 & 11.34\% \\
% 500   & 0.3767 & 0.3468 &  7.94\% \\
% 600   & 0.3981 & 0.3378 & 15.15\% \\
% 700   & 0.3893 & 0.3364 & 13.59\% \\
% 800   & 0.3778 & 0.3641 &  3.63\% \\
% 900   & 0.3619 & 0.3587 &  0.88\% \\
% 1000  & 0.3717 & 0.3550 &  4.49\% \\
%         \bottomrule
%     \end{tabular}
    
%     \end{subtable}



%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Darcy Flow test errors trained on 20 training data size across various sampling density.}}
%         \centering
  
%     \begin{tabular}{rccc}
%         \toprule

%         \textbf{Density}& \textbf{GKN} & \textbf{Ours} & \textbf{Error Reduction} \\
%         \midrule
% 20    & 0.5909 & 0.5363 &  9.24\% \\
% 30    & 0.5712 & 0.5131 & 10.17\% \\
% 40    & 0.5493 & 0.4674 & 14.91\% \\
% 50    & 0.5221 & 0.4445 & 14.86\% \\
% 60    & 0.5013 & 0.4251 & 15.20\% \\
% 70    & 0.4975 & 0.3965 & 20.30\% \\
% 80    & 0.4937 & 0.3709 & 24.87\% \\
% 90    & 0.4920 & 0.3638 & 26.06\% \\
% 100   & 0.4790 & 0.3986 & 16.78\% \\
% 200   & 0.3937 & 0.2812 & 28.58\% \\
% 300   & 0.3414 & 0.2416 & 29.23\% \\
% 400   & 0.3291 & 0.2471 & 24.92\% \\
% 500   & 0.3285 & 0.2247 & 31.60\% \\
% 600   & 0.3030 & 0.2362 & 22.05\% \\
% 700   & 0.3001 & 0.2332 & 22.29\% \\
% 800   & 0.2841 & 0.2303 & 18.94\% \\
% 900   & 0.2787 & 0.2215 & 20.52\% \\
% 1000  & 0.2660 & 0.2297 & 13.65\% \\
%         \bottomrule
%     \end{tabular}

%     \end{subtable}


%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Eikonal test errors trained on 20 training data size across various sampling density.}}
%         \centering

%       \begin{tabular}{cccc}
%         \toprule
%         \textbf{Density} & \textbf{GKN} & \textbf{Ours} & \textbf{Error Reduction} \\
%         \midrule
% 20    & 0.1985 & 0.1543 & 22.27\% \\
% 30    & 0.1941 & 0.1377 & 29.06\% \\
% 40    & 0.1916 & 0.1255 & 34.50\% \\
% 50    & 0.1880 & 0.1191 & 36.65\% \\
% 60    & 0.1864 & 0.1192 & 36.05\% \\
% 70    & 0.1838 & 0.1154 & 37.21\% \\
% 80    & 0.1835 & 0.1170 & 36.24\% \\
% 90    & 0.1847 & 0.1140 & 38.28\% \\
% 100   & 0.1848 & 0.1115 & 39.66\% \\
% 200   & 0.1780 & 0.1069 & 39.94\% \\
% 300   & 0.1757 & 0.1066 & 39.33\% \\
% 400   & 0.1716 & 0.1058 & 38.34\% \\
% 500   & 0.1703 & 0.1060 & 37.76\% \\
% 600   & 0.1739 & 0.1073 & 38.30\% \\
% 700   & 0.1682 & 0.1038 & 38.29\% \\
% 800   & 0.1696 & 0.1038 & 38.80\% \\
% 900   & 0.1705 & 0.1059 & 37.89\% \\
% 1000  & 0.1697 & 0.1059 & 37.60\% \\
%         \bottomrule
%     \end{tabular}
    
%     \end{subtable}

% \end{table*}

% \begin{table*}
    

%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Nonlinear Diffusion test errors trained on 20 training data size across various sampling density.}}
%         \centering

%     \begin{tabular}{cccc}
%         \toprule
%         \textbf{Density} & \textbf{GKN} & \textbf{Ours} & \textbf{Error Reduction} \\
%         \midrule
% 20    & 0.3053 & 0.2403 & 21.29\% \\
% 30    & 0.2804 & 0.2003 & 28.57\% \\
% 40    & 0.2655 & 0.1755 & 33.90\% \\
% 50    & 0.2525 & 0.1661 & 34.22\% \\
% 60    & 0.2459 & 0.1580 & 35.75\% \\
% 70    & 0.2420 & 0.1498 & 38.10\% \\
% 80    & 0.2387 & 0.1401 & 41.31\% \\
% 90    & 0.2313 & 0.1329 & 42.54\% \\
% 100   & 0.2284 & 0.1332 & 41.68\% \\
% 200   & 0.2056 & 0.1060 & 48.44\% \\
% 300   & 0.1923 & 0.0920 & 52.16\% \\
% 400   & 0.1831 & 0.0847 & 53.74\% \\
% 500   & 0.1783 & 0.0826 & 53.67\% \\
% 600   & 0.1780 & 0.0781 & 56.12\% \\
% 700   & 0.1755 & 0.0731 & 58.35\% \\
% 800   & 0.1749 & 0.0728 & 58.38\% \\
% 900   & 0.1755 & 0.0740 & 57.83\% \\
% 1000  & 0.1716 & 0.0757 & 55.89\% \\
%         \bottomrule
%     \end{tabular}
    
%     \end{subtable}



%     \begin{subtable}{\textwidth}
%         \caption{\small \textit{Advection test errors trained on 20 training data size across various sampling density.}}
%         \centering

%     \begin{tabular}{cccc}
%         \toprule
%         \textbf{Density} & \textbf{GKN} & \textbf{Ours} & \textbf{Error Reduction} \\
%         \midrule
% 20    & 1.0704 & 0.5114 & 52.22\% \\
% 30    & 1.0391 & 0.4973 & 52.14\% \\
% 40    & 0.9612 & 0.5189 & 46.02\% \\
% 50    & 0.9652 & 0.5618 & 41.79\% \\
% 60    & 0.8556 & 0.5541 & 35.24\% \\
% 70    & 0.8128 & 0.5524 & 32.04\% \\
% 80    & 0.7770 & 0.5318 & 31.56\% \\
% 90    & 0.8157 & 0.5334 & 34.61\% \\
% 100   & 0.8125 & 0.5498 & 32.33\% \\
% 200   & 0.8552 & 0.5004 & 41.49\% \\
% 300   & 0.7282 & 0.5323 & 26.90\% \\
% 400   & 0.7667 & 0.5317 & 30.65\% \\
% 500   & 1.0101 & 0.5431 & 46.23\% \\
% 600   & 0.7948 & 0.5754 & 27.60\% \\
% 700   & 0.7928 & 0.5594 & 29.44\% \\
% 800   & 0.8037 & 0.4799 & 40.29\% \\
% 900   & 0.7267 & 0.4866 & 33.04\% \\
% 1000  & 0.7421 & 0.5268 & 29.01\% \\
%         \bottomrule
%     \end{tabular}
    
%     \end{subtable}

%     \end{table*}



    
%   %   \begin{subtable}{\textwidth}
%   %       \caption{\small \textit{Test errors  trained on 100 training data size across various sampling density.}}
%   %       \centering

%   % \begin{tabular}{rccc}
%   %   \toprule
%   %   \textbf{traning data size} & \textbf{GKN} & \textbf{OURS} & \(\displaystyle\frac{\mathrm{GKN}-\mathrm{OURS}}{\mathrm{GKN}}\) \\
%   %   \midrule
%   %    20   & 0.5027 & 0.4269 & 0.1507857569 \\
%   %    30   & 0.4746 & 0.3776 & 0.2043826380 \\
%   %    40   & 0.4572 & 0.3328 & 0.2720909886 \\
%   %    50   & 0.4283 & 0.3072 & 0.2827457390 \\
%   %    60   & 0.3995 & 0.2884 & 0.2780976220 \\
%   %    70   & 0.3885 & 0.2864 & 0.2628056628 \\
%   %    80   & 0.3760 & 0.2750 & 0.2686170213 \\
%   %    90   & 0.3646 & 0.2572 & 0.2945693911 \\
%   %   100   & 0.3402 & 0.2519 & 0.2595532040 \\
%   %   200   & 0.2633 & 0.1878 & 0.2867451576 \\
%   %   300   & 0.2355 & 0.1624 & 0.3104033970 \\
%   %   400   & 0.2097 & 0.1485 & 0.2918454936 \\
%   %   500   & 0.2020 & 0.1433 & 0.2905940594 \\
%   %   600   & 0.1911 & 0.1376 & 0.2799581371 \\
%   %   700   & 0.1874 & 0.1349 & 0.2801494130 \\
%   %   800   & 0.1788 & 0.1325 & 0.2589485459 \\
%   %   900   & 0.1777 & 0.1289 & 0.2746201463 \\
%   %  1000   & 0.1748 & 0.1277 & 0.2694508009 \\
%   %   \bottomrule
%   % \end{tabular}
  
%   %   \end{subtable}



%     % \begin{subtable}{\textwidth}
%     %     \caption{\small \textit{Test errors for different models trained on 100 training data size across various PDE benchmarks.}}
%     %     \centering
%     %     \begin{tabular}{lccccc}
%     %         \toprule
%     %         \textit{Dataset} & GCN & DeepONet & FNO & GKN & Ours\\
%     %         \midrule
%     %         Darcy Flow           & 0.6378 & 0.2289 & 0.0645 & 0.1748 & 0.1277 \\
%     %         Advection            & 0.9575 & 0.1691 & 0.1847 & 0.2886 & 0.2350\\
%     %         Eikonal              & 0.1850 & 0.2052 & 0.0523 & 0.1168 & 0.0643 \\
%     %         Nonlinear Diffusion & 0.2474 & 0.1912 & 0.0223 & 0.1044 & 0.0495 \\
%     %         \bottomrule
%     %     \end{tabular}
%     % \end{subtable}



% \end{table*}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points4000_with_training_size.jpg}
%   \caption{Test error trend with sampling density=4000}
% \end{figure}



% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points900_with_training_size.jpg}
%   \caption{Test error trend with sampling density=900}
% \end{figure}



% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points800_with_training_size.jpg}
%   \caption{Test error trend with sampling density=800}
% \end{figure}


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points700_with_training_size.jpg}
%   \caption{Test error trend with sampling density=700}
% \end{figure}


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points600_with_training_size.jpg}
%   \caption{Test error trend with sampling density=600}
% \end{figure}



% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points500_with_training_size.jpg}
%   \caption{Test error trend with sampling density=500}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points400_with_training_size.jpg}
%   \caption{Test error trend with sampling density=400}
% \end{figure}


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points300_with_training_size.jpg}
%   \caption{Test error trend with sampling density=300}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points200_with_training_size.jpg}
%   \caption{Test error trend with sampling density=200}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points100_with_training_size.jpg}
%   \caption{Test error trend with sampling density=100}
% \end{figure}


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points90_with_training_size.jpg}
%   \caption{Test error trend with sampling density=90}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points80_with_training_size.jpg}
%   \caption{Test error trend with sampling density=80}
% \end{figure}


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points70_with_training_size.jpg}
%   \caption{Test error trend with sampling density=70}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points60_with_training_size.jpg}
%   \caption{Test error trend with sampling density=60}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points50_with_training_size.jpg}
%   \caption{Test error trend with sampling density=50}
% \end{figure}


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points40_with_training_size.jpg}
%   \caption{Test error trend with sampling density=40}
% \end{figure}


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points30_with_training_size.jpg}
%   \caption{Test error trend with sampling density=30}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/test_points20_with_training_size.jpg}
%   \caption{Test error trend with sampling density=20}
% \end{figure}


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/error_heatmap_with_train_100.jpg}
%   \caption{Error Reduction Heatmap with Train Data Size=100}
% \end{figure}


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/error_heatmap_with_train_50.jpg}
%   \caption{Error Reduction Heatmap with Train Data Size=50}
% \end{figure}



% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/error_heatmap_with_train_40.jpg}
%   \caption{Error Reduction Heatmap with Train Data Size=40}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/error_heatmap_with_train_30.jpg}
%   \caption{Error Reduction Heatmap with Train Data Size=30}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/error_heatmap_with_train_20.jpg}
%   \caption{Error Reduction Heatmap with Train Data Size=20}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/error_heatmap_with_train_10.jpg}
%   \caption{Error Reduction Heatmap with Train Data Size=10}
% \end{figure}




% % \subsection{Generalization across point density}



% % % \begin{table*}[h]
% % % % \caption{\small training data size is 100, test data size is 100, sample points is 200 }
% % %     \small
% % %     \centering


% % %     \begin{subtable}{\textwidth}
% % %     \caption{\small \textit{training data size is 100, test data size is 100, sample points is 20}}
% % %     \small 
% % %     \centering
% % % \begin{tabular}{cccc}
% % %     \hline
% % %     \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %     Darcy Flow                  &  & 0.5027	& 0.4269       \\
% % %     Advection   &  & 0.9035	& 0.3980      \\
% % %     Eikonal            &  & 0.1808      & 0.1236 \\
% % %     Nonlinear Diffusion            &  & 0.2407    & 0.2030 \\
% % %      \hline
% % % \end{tabular}
% % % \end{subtable}  




% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 100, test data size is 100, sample points is 100}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.3402	& 0.2519         \\
% % %         Advection   &  & 0.3446	& 0.3216        \\
% % %         Eikonal            &  & 0.1442        & 0.0857   \\
% % %         Nonlinear Diffusion            &  & 0.1689      & 0.1099 \\
% % %         Poisson            &  & 0.3529        &    0.3402 
        
% % %         \\ \hline
% % %     \end{tabular}
% % %     \end{subtable}  

    
% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 100, test data size is 100, sample points is 200}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.2633	& 0.1878         \\
% % %         Advection   &  & 0.3150	& 0.2880         \\
% % %         Eikonal            &  & 0.1325        & 0.0745   \\
% % %         Nonlinear Diffusion            &  & 0.1415      & 0.0855 \\
% % %         Poisson            &  & 0.2943        &    0.2753 
        
% % %         \\ \hline
% % %     \end{tabular}
% % %     \end{subtable}  


% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 100, test data size is 100, sample points is 300}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.2355	& 0.1624         \\
% % %         Advection   &  & 0.3017	& 0.2537        \\
% % %         Eikonal            &  & 0.1238       & 0.0664   \\
% % %         Nonlinear Diffusion            &  & 0.1245      & 0.0751 \\
% % %         Poisson            &  & 0.2645       &    0.2424 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}  


% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 100, test data size is 100, sample points is 400}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.2027	& 0.1485        \\
% % %         Advection   &  & 0.3005	& 0.2516       \\
% % %         Eikonal            &  & 0.1203       & 0.0669   \\
% % %         Nonlinear Diffusion            &  & 0.1118      & 0.0687 \\
% % %         Poisson            &  & 0.2448       &    0.2249 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}  


% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 100, test data size is 100, sample points is 500}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.2020	& 0.1433        \\
% % %         Advection   &  & 0.2997	& 0.2462       \\
% % %         Eikonal            &  & 0.1209       & 0.0671   \\
% % %         Nonlinear Diffusion            &  & 0.1115      & 0.0637 \\
% % %         Poisson            &  & 0.2337       &    0.2080 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}  


% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 100, test data size is 100, sample points is 600}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.1911	& 0.1376        \\
% % %         Advection   &  & 0.2868	& 0.2453       \\
% % %         Eikonal            &  & 0.1199       & 0.0665  \\
% % %         Nonlinear Diffusion            &  & 0.1093     & 0.0623 \\
% % %         Poisson            &  & 0.2191       &    0.2010 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}  


% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 100, test data size is 100, sample points is 700}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.1874	& 0.1349        \\
% % %         Advection   &  & 0.2972	& 0.2421      \\
% % %         Eikonal            &  & 0.1159       & 0.0676  \\
% % %         Nonlinear Diffusion            &  & 0.1101     & 0.0544 \\
% % %         Poisson            &  & 0.2126       &    0.1923 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}










% % % \end{table*}


% % % \begin{table*}[h]
% % % % \caption{\small training data size is 100, test data size is 100, sample points is 200 }
% % %     \small
% % %     \centering

% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 100, test data size is 100, sample points is 800}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.1788	& 0.1325        \\
% % %         Advection   &  & 0.3083	& 0.2408      \\
% % %         Eikonal            &  & 0.1148      & 0.0665  \\
% % %         Nonlinear Diffusion            &  & 0.1073    & 0.0527\\
% % %         Poisson            &  & 0.2067       &    0.1870 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}

    

% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 100, test data size is 100, sample points is 900}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.1777	& 0.1289       \\
% % %         Advection   &  & 0.2926	& 0.2310      \\
% % %         Eikonal            &  & 0.1173      & 0.0655  \\
% % %         Nonlinear Diffusion            &  & 0.1054    & 0.0522\\
% % %         Poisson            &  & 0.2028       &    0.1794 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}


    

% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 100, test data size is 100, sample points is 1000}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.1748	& 0.1277       \\
% % %         Advection   &  & 0.2886	& 0.2350      \\
% % %         Eikonal            &  & 0.1168      & 0.0643 \\
% % %         Nonlinear Diffusion            &  & 0.1044    & 0.0495\\
% % %         Poisson            &  & 0.1980       &    0.1749 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}

    
% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 100, test data size is 100, sample points is 1100}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.1669	& 0.1235       \\
% % %         Advection   &  & 0.2919	& 0.2375      \\
% % %         Eikonal            &  & 0.1187      & 0.0670 \\
% % %         Nonlinear Diffusion            &  & 0.1013    & 0.0490\\
% % %         Poisson            &  & 0.1978      &    0.1686 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}

% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 100, test data size is 100, sample points is 1200}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.1604	& 0.1223       \\
% % %         Advection   &  & 0.2923	& 0.2414      \\
% % %         Eikonal            &  & 0.1147      & 0.0666 \\
% % %         Nonlinear Diffusion            &  & 0.1012    & 0.0477\\
% % %         Poisson            &  & 0.1901      &    0.1617 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}

% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 100, test data size is 100, sample points is 1300}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.1604	& 0.1223       \\
% % %         Advection   &  & 0.2923	& 0.2414      \\
% % %         Eikonal            &  & 0.1147      & 0.0666 \\
% % %         Nonlinear Diffusion            &  & 0.1012    & 0.0477\\
% % %         Poisson            &  & 0.1901      &    0.1617 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}

    
% % % \end{table*}




% % % \begin{table*}[h]
% % % % \caption{\small training data size is 100, test data size is 100, sample points is 200 }
% % %     \small
% % %     \centering

    

% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 50, test data size is 100, sample points is 100}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.4068	& 0.2918       \\
% % %         Advection   &  & 0.4467	& 0.4130      \\
% % %         Eikonal            &  & 0.1592      & 0.0988 \\
% % %         Nonlinear Diffusion            &  & 0.1903    & 0.1157\\
% % %         Poisson            &  & 0.3826      &    0.3647 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}


% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 50, test data size is 100, sample points is 1000}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.1890	& 0.1597       \\
% % %         Advection   &  & 0.3717	& 0.3550      \\
% % %         Eikonal            &  & 0.1273      & 0.0895 \\
% % %         Nonlinear Diffusion            &  & 0.1218    & 0.0602\\
% % %         Poisson            &  & 0.3826      &    0.3647 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}


% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 30, test data size is 100, sample points is 100}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.4404	& 0.3705       \\
% % %         Advection   &  & 0.5708	& 0.4977      \\
% % %         Eikonal            &  & 0.1825      & 0.1047 \\
% % %         Nonlinear Diffusion            &  & 0.2168    & 0.1414\\
% % %         Poisson            &  & 0.3788      &    0.3807 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}


% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 30, test data size is 100, sample points is 1000}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.4404	& 0.3705       \\
% % %         Advection   &  & 0.5708	& 0.4977      \\
% % %         Eikonal            &  & 0.1825      & 0.1047 \\
% % %         Nonlinear Diffusion            &  & 0.2168    & 0.1414\\
% % %         Poisson            &  & 0.3788      &    0.3807 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}


% % %     \begin{subtable}{\textwidth}
% % %         \caption{\small \textit{training data size is 30, test data size is 100, sample points is 1000}}
% % %         \small 
% % %         \centering
% % %     \begin{tabular}{cccc}
% % %         \hline
% % %         \textit{Dataset}      &  & Baseline             & Ours            \\ \hline
% % %         Darcy Flow                  &  & 0.4404	& 0.3705       \\
% % %         Advection   &  & 0.5708	& 0.4977      \\
% % %         Eikonal            &  & 0.1825      & 0.1047 \\
% % %         Nonlinear Diffusion            &  & 0.2168    & 0.1414\\
% % %         Poisson            &  & 0.3788      &    0.3807 \\
% % %          \hline
% % %     \end{tabular}
% % %     \end{subtable}
    
    
% % % \end{table*}
    



% % \section{Conclusion}



% \newpage

% \bibliographystyle{apalike}



% \bibliography{ref}   



% \end{document}

==> related.tex <==
\section{Related Work}

% \subsection{Operator Learning for PDEs}
% Operator learning frameworks, such as DeepONet \citep{lu2019deeponet} and Fourier Neural Operator (FNO) \citep{li2020fourier}, have pioneered learning mappings between infinite-dimensional function spaces. DeepONet uses a branch–trunk neural network to approximate solution operators, while FNO leverages Fourier transforms for efficient learning in spectral space. These approaches demonstrate strong performance on structured data but often assume regular discretizations.
% Both DeepONet and FNO rely on fixed, structured grids, making them ill-suited for PDE problems defined on irregular geometries or sparse, adaptive point clouds. FNO, in particular, depends on the fast Fourier transform (FFT), which assumes periodic, Euclidean grids and suffers performance degradation under non-uniform sampling.


% \subsection{Graph Neural Networks for Scientific Machine Learning}

There are many latest research about graph and attention methods in scientific machine learning \citep{pmlr-v235-xiao24c}, \cite{kissas2022learning}, \cite{boulle2024mathematical}, \cite{xu2024equivariant}, \cite{jin2023leveraging},
\cite{cuomo2022physics}
\cite{kovachki2024operator},
\cite{nelsen2024operator},
\cite{batlle2023kernel}.

\textbf{Graph neural networks for scientific machine learning.} \cite{battaglia2018relational} applies shared functions over nodes and edges, captures relational inductive biases and generalizes across different physical scenarios.
\cite{barsinai2019learning} learns data-driven discretization schemes for solving PDEs by training a neural network to predict spatial derivatives directly from local stencils. By replacing hand-crafted finite difference rules with learned operators, it adapts discretizations to the underlying data for improved accuracy and generalization.
\cite{sanchezgonzalez2020learning} predicts future physical states by performing message passing over the mesh graph, capturing both local and global dynamics without relying on explicit numerical solvers.
 Graph Kernel Networks (GKNs) \citep{li2020neural} directly approximates continuous mappings between infinite-dimensional function spaces by utilizing graph kernel convolution layers.
PDE-GCN \citep{wang2022pdegcn} represents partial differential equations on arbitrary graphs by combining spectral graph convolution with PDE-specific inductive biases. It learns to predict physical dynamics directly on graph-structured domains, enabling generalization across varying geometries and discretizations.
The Message Passing Neural PDE Solver \citep{brandstetter2022message} 
 formulates spatiotemporal PDE dynamics by applying learned message passing updates on graph representations of the solution domain.
Physics-Informed Transformer (PIT) \citep{zhang2024attention} embeds physical priors into the Transformer architecture to model PDE surrogate solutions. It leverages self-attention to capture long-range dependencies and integrates PDE residuals as soft constraints during training to improve generalization.
GraphCast \citep{lam2024graphcast} learns the Earth’s atmosphere as a spatiotemporal graph and uses a graph neural network to iteratively forecast future weather states based on past observations. It performs message passing over the graph to capture spatial correlations and temporal dynamics, enabling accurate medium-range forecasts.


% \subsection{Attention-Based Methods for Scientific Machine Learning}

\textbf{Attention-based methods for scientific machine learning.}
U-Netformer \citep{liu2022unetformer} proposes a hybrid neural architecture that combines the U-Net's hierarchical encoder-decoder structure with transformer-based attention modules to capture both local and global dependencies in PDE solution spaces. 
Tokenformer \citep{zhou2023tokenformer} reformulates PDE solving as a token mixing problem by representing input fields as tokens and applying self-attention across them to model spatial correlations.
Tokenized Neural Operators (TNO) \citep{jiang2023tokenized} framework reformulates operator learning as a token-wise attention problem, where spatial inputs are encoded into tokens and processed using Transformer-style architectures. It employs a combination of axial attention and cross-attention to efficiently capture both local and global dependencies across irregular or structured domains.
Attention-Based Fourier Neural Operator (AFNO) \citep{zhang2024attention} enhances the standard FNO by integrating self-attention layers after each Fourier convolution block to better capture local dependencies and long-range interactions. This hybrid architecture improves the model’s ability to approximate complex solution operators for parametric PDEs by combining spectral global context with spatial attention mechanisms.



Our proposed GOLA combines the local relational strengths of attention-enhanced GNNs and the global spectral capabilities of Fourier-based encoding. This hybrid approach has shown notable improvements in generalization and data efficiency, particularly under challenging data-scarce conditions on irregular domains.




